Knowing-how & Knowing-that: A New Task for Machine Comprehension of User Manuals

The machine reading comprehension (MRC) of user manuals has huge potential in customer service. However, current methods have trouble answering complex questions. Therefore, we introduce the Knowing-how & Knowing-that task that requires the model to answer factoid-style, procedure-style, and inconsistent questions about user manuals. We resolve this task by jointly representing the steps and facts in a graph TARA, which supports a unified inference of various questions. Towards a systematical benchmarking study, we design a heuristic method to automatically parse user manuals into TARAs and build an annotated dataset to test the model's ability in answering real-world questions. Empirical results demonstrate that representing user manuals as TARAs is a desired solution for the MRC of user manuals. An in-depth investigation of TARA further sheds light on the issues and broader impacts of future representations of user manuals. We hope our work can move the MRC of user manuals to a more complex and realistic stage.

==> chapters-old/Experiments_v1.tex <==
\newcommand{\ourmodel}{\textit{GraphMatch}\xspace}

\section{Experiments}

\input{tables/exp1}
\subsection{Evaluation metrics}Based on the answer type, we leverage four types of metrics. For \texttt{Q1} and \texttt{Q4}, we introduce the BLEU-based precision, recall and F1 scores~\cite{tandon-etal-2020-dataset}, denoted as P$^\dag$, R$^\dag$, and F1$^\dag$, respectively. For \texttt{Q2} and \texttt{Q5}, we compute the P$^\dag$, R$^\dag$, and F1$^\dag$ scores of each element in a n-tuple, and report the average score of these elements. For \texttt{Q3}, we borrow the idea of measure pairwise strings and compute the Hamming distance~(HD) and Levenshtein distance~(LD) between the predicated action lists and the gold ones. For \texttt{Q6} and \texttt{Q7}, we report the classic precision, recall and F1 scores, denoted as P, R, and F1, respectively. Higher values of P$^\dag$, R$^\dag$, F1$^\dag$, P, R, and F1 indicate the better performance. On the contrary, lower values of HD and LD indicate the better performance.
\subsection{Results} 
\label{sec:results}
From Table~\ref{tab:exp1}, we can see that:
\begin{itemize}
    \item It is challenging to make an integrated comprehension of user instructions. Although there is a clear rank of these approaches, the gap between the best results and the worst ones on all metrics is not significant. What's more, even the best results of the baseline approaches still far behind the human upper bound.
    \item The declaration first strategy is slightly better than the procedure first strategy. The two strategies are expected to work equally better if the semantic dependency are correctly parsed. We conjecture the unexpection is caused by the frequently missing agents~(i.e., the user entity) in procedure. This makes the model fail to detect actions that should be taken by users. Hence, the approach using procedure first strategy get lower precision scores compared to the one using declaration first strategy. Another possible cause is the long sentence issue. If the agent of the core predicate is user, the parser usually uses it as agents for the predicates without agents in the sentence. In other words, the parser tends to over-produce actions. As a result, the approach using procedure first strategy get lower recall scores compared to the one using declaration first strategy
    \item Better semantic dependency parsing tools produce better results. 
    LTP-\kts stands out of the other approaches with half first places on all metrics. LTP-\khs ranks the second with the most second best results. In most cases, the models with Biafiine as the backbone parse are at the low-ranking places, except for the LD metrics on \texttt{Q3}. With a close look at the parsed results. we find this is because the Biafiine parser produces about four actions for each procedure on average. The number is much more similar to the gold results than the other models that over-produces actions. As a result, the approaches with Biafiine as the backbone parse obtain the best LD scores.
    \item %Error propagation matters for the results.  
    The cascading errors damage the performance.The results of \texttt{Q2} and \texttt{Q3} depend on\texttt{Q1}. The results of \texttt{Q5} depend on \texttt{Q4}. The results of \texttt{Q6} and \texttt{Q7} depend on all the other questions and suffer the most from cascading errors. This explains why all baseline approaches produce similar results on all metrics of \texttt{Q6} and \texttt{Q7}.
\end{itemize}
%   Wat's
% LTP-\kts stands out of the other approaches with half first places on all metrics.  This indicates that using a better semantic dependency parser is likely to get better performance.
\subsection{Experiment \Rmnum{2}: QA on real-world questions}
\paragraph{Experiment setting.} Experiment \Rmnum{1} has a strong assumption that the system can perfectly comprehend the question. This is not always reachable in real-world scenarios. Thus, we further conduct the QA task on real-world questions. We obtain the customer service logs of the e-commerce company and randomly collect 100000 questions containing the entities in the annotated user instructions. We rank the questions based on the BM25 scores with the annotated user instructions and keep the top 2500 questions. Then, we invite the staff from the marketing department to manually check whether the questions are related to the user instructions or not. If the question is related to the user instruction, we further ask the staff to provide the answers based on corresponding document. Finally, we get 2052 real-world Q-A pairs on the user instructions. 

After an examination of the real-world questions, we find that the percentage of the three question types~(cf., Sec. ~\ref{sec:task_rep}) are 50\%, 25\%, and 25\%, respectively. In other words, the \texttt{T3} questions govern the real-word custom service. Thus, in this experiment, most of the answers are potential evidence for \texttt{T3} questions. \par

To perform the QA task, we build an unsupervised QA model called \ourmodel using parsed user instructions and semantic parsing tools. And we compare it with various other types of unsupervised QA models. We build our QA model using the LTP tool for question parsing and reason over the parsed user instructions to find the final answers.

Specifically, we first utilize the parsing tool to parse the question into a dependency semantic representation to obtain the core predicate described by the question and corresponding object. Then we use simple heuristic rules to divide questions into questions asking for a step and questions asking for an entity. For the question of asking the step, we match it with the most relevant step in the procedure. For the question of asking the entity, we match it with the most relevant entity in the declaration. We obtain the best match through the similarity score between the core predicate and object of the question and the action and patient of the step in the procedure. Similarly, we obtain the best match between the question object and the entity in the declaration in the same way. Both similarity scores are obtained by calculating the Edit Distance score between corresponding text strings of questions and procedural or declarative information. The specific calculation for the score is shown in Formula 1: 
\begin{equation}
1-\frac{EditDistance(tq, tg)}{max(len(tq), len(tg))}
\end{equation}
where $EditDistance(tq, tg)$ calculates the edit distance between the question text and the candidate answer and $max(len(tq), len(tg))$ calculates the maximum length of string for the question text and the candidate answer. 

Then, we judge the focus of the question through the arguments obtained from the question parsing and find the corresponding argument in the step as the answer. If no corresponding argument is found in the current step, the search will be repeated in the previous one, and the search can be conducted in the previous two steps at most. In particular, for inconsistent questions, we take the entity information linked by the arguments in the current step as the candidate answers. For the question of asking the entity, we return the sentence containing the corresponding entity information in the declaration.
An example of the reasoning process by \ourmodel is shown in Figure~\ref{fig:example}, the inference path is highlighted in black.

To prove the effectiveness of the proposed structured knowledge by us and the QA model \ourmodel based on it, we compare our model with other types of unsupervised QA models on this real-world data set. The unsupervised QA baselines we selected for comparison are listed as follows:\\
\\
\textbf{SurfacePatternMatching}
\begin{itemize}
    \item \textbf{User Instruction Pattern}: Surface Pattern based matching algorithm uses handwritten rules to match questions and answers with corresponding syntactic formats\cite{ravichandran2002learning, soubbotin2001patterns, greenwood2003using}. This approach has high accuracy, but the recall rate is low because it completely depends on the fixed sentence syntax.
\end{itemize}
\hfill\break
\textbf{LexicalMatching}
Lexical Matching approaches compare the similarity between the question text and the candidate answer in terms of lexical features. Therefore, we can find the sentences that literally match the question description as the final answer.
\begin{itemize}
    \item \textbf{BLEU}: Bleu is often used to measure the lexical similarity between texts. It can be used to compare the similarity between question and candidate answers in QA to find the best answer\cite{alfonseca2001prototype}. In addition, we give higher reward points to the candidate answers containing the entities mentioned in the question\cite{yang2018adaptations} for better matching.
    \item \textbf{Levenshtein Distance}: Levenshtein Distance is a common indicator used to measure the lexical gap between texts. We also use the transformation shown in Formula 1 to calculate the lexical similarity between question and candidate answers\cite{coates2022identifying}.
\end{itemize}
\hfill\break
\textbf{SemanticMatching}
In addition to lexical level matching, comparing the similarity between question and candidate answers semantically can better mine the potential semantic information of the text and achieve more accurate matching.
\begin{itemize}
    \item \textbf{Bert Base}: Use the attention mechanism to collect information about the context of words, and encode it with a rich vector representing the context\cite{devlin2018bert}.
    \item \textbf{Char CNN}: Text encoding model based on character level granularity which can deal with typographical errors and avoid OOV problem\cite{zhang2015character}.
    \item \textbf{Chinese Word Vectors}: A sparse Chinese pre-training word vector containing different context features (words, N-tuples, characters, etc.)\cite{P18-2023}.
    \item \textbf{Bert Score}: Leveraging the pre-trained contextual embeddings from BERT and matching words in candidate and reference sentences by cosine similarity\cite{bert-score}.
\end{itemize}
\hfill\break
\textbf{KeywordsMatching}
Keywords Matching determines the best matching answer by comparing the co-occurrence of keywords in question and candidate answers.
\begin{itemize}
    \item \textbf{Synonyms Plus}: Get as many keywords in the question as possible by rewriting the question and replacing synonyms. Then match them with the keywords in the candidate answers to calculate the similarity score\cite{katyayan2022design}.
    \item \textbf{Keywords Window}: In addition to keywords co-occurrence, the farthest distance between keywords of question in candidate answers and the syntactic similarity between keywords in question and answer are taken into account\cite{moldovan2000structure}.
\end{itemize}
\hfill\break
\textbf{Pre-trainingLanguageModel}
The pre-training language model is pre-trained on large-scale MRC datasets and can be directly used for Question Answering without fine-tuning on downstream tasks.
\begin{itemize}
    \item \textbf{Macbert Large}: MLM as correction, using correction as the language model of the mask, reduces the gap between pre-training and fine-tuning stages by using similar words mask\cite{cui2020revisiting}.
    \item \textbf{Pert Large}: A pre-training model based on a disordered language model, which can self-supervise the learning of text semantic information without introducing mask tags\cite{cui2022pert}.
    \item \textbf{Roberta wwm}: Based on BERT's language masking strategy, using dynamic masks and a larger byte level BPE vocabulary for training\cite{liu2019roberta}.
\end{itemize}
\hfill\break
\textbf{SelfSupervised}
Taking advantage of the potential QA pairs mined from the text to construct the dataset for training is a self-supervised learning approach\cite{baralunsupervised, nie2022unsupervised}. It can obtain a large amount of data without manual annotation to fine-tune the pre-training model. Inspired by previous work\cite{lewis2019unsupervised}, we mask corresponding arguments in the document sentences and replace them with interrogative words (when, where, why, how, etc.) to construct QA data. We finally constructed 800000 QA pairs from 360000 documents as the dataset for model training. The models we use for fine-tuning are the three pre-training models mentioned above: Macbert\cite{cui2020revisiting}, Pert\cite{cui2022pert} and Roberta\cite{liu2019roberta}.

\paragraph{Evaluation metrics} We use standard BLEU and F1 metrics to evaluate the Question Answering results. Note that, pre-training language models and self-supervised models can only produce one consecutive span, but \ourmodel and other proposed baselines can produce multiple evidence via inference. Therefore, to make a fair comparison, we conducted an additional experiment in which we set the answer's hit ratio as 1 for all models. More importantly, we evaluated the question matching rate of the Surface Pattern Matching model and \ourmodel, indicating the correct rate of their heuristic rules to the question identification, to ensure that they can correctly identify most questions.
\paragraph{Results.}
\input{tables/QA_result.tex}
We evaluated all models on the labeled QA data set, and the results are shown in Table~\ref{tab:exp2}. From the results, we can see that the model \ourmodel proposed by us can more accurately perceive the actions and related entity information required for the specific step mentioned in the question. This gets benefits from our approach which models the information of procedural and declarative in the document and the relationship between them. 
For Surface Pattern Matching, even though our manually written templates can match most of the questions, the overall recall rate is low due to the flexible answer sentence structures and the lack of reasoning ability. 
For Lexical Matching and Semantic Matching approaches, pure lexical and semantic similarity matching ignores the important role of the core predicate in answer reasoning, and this kind of method can not link related entity information with corresponding steps in procedures. 
Keywords Matching algorithms focus on nominal keywords information in question and candidate answers, but important predicate information and arguments information related to core operation are ignored. 
Pre-training language models have poor performance due to the difference between the pre-training corpus and the target data set. 
After fine-tuning on the constructed data set, the performance of the models has been significantly improved. However, because the constructed training data only aims at the factoid style questions and they do not have the ability to reason between procedural and declarative information, the final performance is still poor.
The excellent performance of our proposed model shows the importance of procedural and declarative information modeling in user instructions and the effectiveness of grasping the relationship between them for supplementing additional evidence.

==> chapters-old/abstract-1225.tex <==
\begin{abstract}
The machine comprehension of user manuals has huge potential in smart customer service. However, current factoid- and procedure-style comprehension models
% overlooked declarative knowledge binding the procedure. This makes the machine 
have trouble answering complex questions~(such as inconsistent questions). 
% In this paper,
% we are interested in a more advanced comprehension of user manuals in the customer service scenario. To this end, 
Thus, we move forward to the machine comprehension of user manuals beyond factoid-style and procedure-style questions. Specifically, we provide the \kh \& \kt benchmark, which is equipped with a real-world corpus from an e-commercial platform, dense annotations of questions and manuals, an efficient baseline based on semantic parsing, and systematical evaluations. 
% To establish it, we collect a real-world corpus from an e-commercial platform, annotate two datasets for extrinsic and intrinsic testing, and design a heuristic baseline.
The extrinsic evaluation results reveal that the integrated comprehension of procedural and declarative knowledge can significantly advance the machine’s intelligence to answer various questions
% , especially complex ones, 
about user manuals. Through the intrinsic results, we further point out that it is still challenging for the machine to do human-level comprehension due to the co-reference issue, etc. We hope to offer a good chance to take forward the study on machine comprehension of user manuals, at least in customer service scenarios.   
% ~(\dataname) and annotate two datasets~(\dataname-E and \dataname-I) based on FAQs and seed questions. We also design a heuristic baseline and test it in both extrinsic and intrinsic settings via \dataname-E and \dataname-I, respectively   
% y collecting a real-world corpus and annotating two datasets, we perform extrinsic and intrinsic evaluations for the machine comprehension of user manuals. 
% {\color{red}
%     The benchmark is equipped with a new corpus with xxx real-world questions about xxx user manuals from an e-commerce platform, a test set with xxx densely annotated question-answer pairs about xxx user manuals, an unsupervised but effective comprehension architecture, and two standard evaluation methods.
% }
% Experimental results reveal the significant challenges of the proposed benchmark and suggest that the integrated comprehension of procedural and declarative knowledge can significantly advance the machine’s intelligence in answering complex questions about user manuals. 
% By human analysis, we describe how the proposed corpus and test set can be used to advance the study of understanding user manuals for smart customer service. We
% further point out the future challenges~(e.g., the co-reference issue) of the proposed benchmark.

% However, the overlook of the declarative knowledge binding procedures presents challenges for current service bots to answer more complex questions~(e.g., inconsistent questions) than factoid-style and procedure-style questions.

% However, in off-the-shelf solutions, the overlook of the declarative knowledge binding procedures
% , as it will enable the machine to answer questions from users

% The automated comprehension of user instruction has huge potential as it contributes to a wide range of applications~(e.g., goal-oriented searching, QA beyond facts). In existing solutions, the procedural knowledge of user instruction is intensively studied, but the declarative knowledge binding procedures is often overlooked. This makes the machine fail to answer more complex questions~(e.g., inconsistent questions) than factoid-style and procedure-style questions. In this paper, we propose a novel benchmark that requires the machine to fully understand a user instruction and answer complex questions about it. 
% {\color{red}
% The benchmark is equipped with a new corpus (\texttt{HeDo}) of helping documents, a hand-annotated test set, and two standard evaluation methods.
% }
% Experimental results reveal the significant challenges of our benchmark and suggest that the integrated comprehension of procedural and declarative information can significantly advance the machine’s intelligence over user instructions. By human analysis, we further point out the future challenges~(e.g., the co-reference issue) of the proposed benchmark.

% Current reading comprehension solutions are largely devoted to procedure comprehension~(\kh) for factoid-style and procedure-style questions. The overlook of declarative knowledge makes them fail to answer more complex questions~(e.g., inconsistent questions). We believe the integrated comprehension of procedural information and declarative information can significantly advance the machine’s intelligence in handling user instructions. In practice, we propose a new benchmark for user instruction comprehension that requires the system to answer factoid-style, procedure-style, and inconsistent questions. This benchmark involves a new corpus (HeDo) of helping documents equipped with a hand-annotated test set, eight baseline approaches, and a standard evaluation method. Experimental results reveal the significant challenges of our benchmark. By human analysis, we further point out the issues in the current study.


% % {\color{red}
% User instruction, with both procedural and declarative information, is widespread infiltrating in our everyday life and has a broad range of applications. However, we argue current solutions to user instructions are not enough for human-level comprehension. Because they are largely devoted to procedure comprehension~(\kh) for factoid-style and procedure-style questions. The overlooking of declaration comprehension~(\kt) doesn't meet Gilbert Ryle's thought that the possession of \kh and \kt is ``a mark of intelligence''. It also makes the system fail to answer inconsistent questions~(i.e., the questions that the user raises when coming across unexpected cases from the instruction). 
% We believe the integrated comprehension of procedural information and declarative information can significantly advance the system’s intelligence in handling user instructions. In practice, we propose a new benchmark for user instruction comprehension that requires the system to answer factoid-style, procedure-style, and inconsistent questions. This benchmark involves a new corpus (HeDo) of helping documents equipped with a hand-annotated test set, eight baseline approaches, and a standard evaluation method. Experimental results reveal the significant challenges of our benchmark. By human analysis, we further point out the issues in the current study.


% ``What is knowledge?'' is a deep philosophical question. One of the classical answers is that the knowledge involves ``\textit{knowing that}'' and ``\textit{knowing how}''. Current knowledge extraction techniques are primarily interested in ``\textit{knowing that}'' --- detecting facts or static events. They seldom venture into ``\textit{knowing how}'' --- the practical side of a concept, e.g., how to make Kung Pao Chicken.
% This heavily holds us back to grasp a whole picture of knowledge and leads to ``vicious regresses''. In this paper, we espouse the philosophers' arguments that it is important to analyze both ``\textit{knowing that}'' and ``\textit{knowing how}''. In keeping with this, we propose a new task to extract ``\textit{knowledge-that}'' and ``\textit{knowledge-how}'' from manuals. We prefer manuals because a manual is always expected to contain the characteristics/requirements~(``\textit{knowledge-that}'') and the handling~(``\textit{knowledge-how}'') of its owner~(food, activity, etc.). We benchmark this task with a hand-annotated dataset, a series of baselines and a set of metrics. Specifically, \textcolor{red}{xxx}. We believe this benchmark can benefit further research. We also hope our work can advance the epistemology, at least in NLP domain, of ``\textit{knowledge-that}'', ``\textit{knowledge-how}'', and how they are grounded. 
% }

% The possession of knowledge-that and knowledge-how is a mark of intelligence.
\end{abstract} 




==> chapters-old/abstract.tex <==
\begin{abstract}

%sell dataset: problem is important but difficult --> we propose a dataset to study this problem --> we propose a method to benchmark this task -- > experiment reveal the task is challenging plus some insight/in-depth analysis.

% 现在问题：structure annotation的重要性没有显示出来。

 The machine reading comprehension~(MRC) of user manuals has huge potential in smart customer service. However, current methods have trouble answering complex questions. Therefore，we propose the \kh \& \kt task to study the MRC of user manuals in a challenging setting, where factoid-style, procedure-style, and inconsistent questions are involved. 
% Wenqiang：automatically represrnt user manuals and questions as heterogeneous graphs。。那就是在突出automatic parsing哦？那定义结构是contribution吗？
To resolve this task, we automatically represent user manuals and questions as heterogeneous graphs to support a unified inference about various questions. We further contribute to a novel dataset~(\dataname) derived from real-world customer service scenarios with 
 careful annotations of FAQs and user manuals. 
% Wenqiang： experiment先reveal advantage再reveal challenge更好。
 Experiments on \dataname reveals the challenges of \kh \& \kt and superiority gained by the joint representation of steps and facts. We hope our work can offer a good chance to move forward with the study on the MRC of user manuals, at least in customer service scenarios.   
 
 
 
 % We construct a unified inference of different questions about the user manual by representing them as heterogeneous graphs. The graphs can be automatically constructed by a novel heuristic method~(HUM) based on several efficient rules. We also contribute to careful annotations for systematical evaluations of question-answering and representation construction. We find that the joint representation of steps and facts can significantly advance the model’s ability to answer various questions about user manuals. Through the empirical results, we further point out that there is still a large margin for the machine to do human-level comprehension. We hope our work can offer a good chance to move forward with the study on machine comprehension of user manuals, at least in customer service scenarios.   
\end{abstract} 




==> chapters-old/base.tex <==
    \begin{figure}[t]
        \centering
        \includegraphics[width=0.5\textwidth]{figures/off.png}
        \caption{The elimination and combination of nodes}
        \label{fig:off}
    \end{figure}
\section{The HUM Method}
\label{sec:AE}
To lay the foundation of the proposed benchmark, we design a fast and robust framework to parse the user instructions like the annotated ones. The framework is based on a pre-trained semantic dependency parsing model and heuristic rules. Given the ordered sentences\footnote{We replace ``you'' and ``your'' with ``user'' and ``user's'' in the sentences, respectively.} of a user instruction, the framework aims to parse the user instruction into steps, entity trees and the groundings defined in Sec.~\ref{sec:task_rep} in a pipeline manner.

\paragraph{1) Parse sentence-level semantic dependency.} We get the sentence-level semantic dependency using a pre-trained semantic dependency parsing model. After that,
\begin{itemize}
    \item If the sentence is imperative, we assign the user entity to the agent of the core predicate. For instance, ``Sign in the APP'' is modified as ``User sign in the APP''.
    \item Given a predicate, except for its agent, the offsprings of its child are eliminated and combined to the child to compose a meaningful phrase, as shown in Figure~\ref{fig:off}

\end{itemize}

\paragraph{2) Get the actions and entities of a procedure.}We propose two strategies~(procedure-first and declaration-first) to get the steps and entities of a procedure. 
\begin{itemize}
    \item The procedure-first strategy assumes that the actions are the consecutive predicates whose agents are user and the entities are extracted from the rest part. 
    \item The declaration-first strategy assumes the entities are the non-user agents or agents labeled as ``EXP'' to the predicates and the actions are extracted from the rest part.
\end{itemize}
If two procedures share at least one predicate and its patient, we combine them into a new procedure, as shown in Figure~\ref{fig:merge}.
        \begin{figure}[t]
        \centering
        \includegraphics[width=0.5\textwidth]{figures/merge.png}
        \caption{The combination of two procedures on the shared predicate and its patient.}
        \label{fig:merge}
    \end{figure}
The alignment from the labels of procedure and declaration to semantic dependency and is presented in Tables~\ref{tab:alig_kh} and \ref{tab:alig_kt}, respectively.
\input{tables/align}
\paragraph{3) Ground the entities and states to procedure.}The user entity is linked to all steps in the procedure by default. The entity is linked to the argument of an action if itself or its sub-entities are seen in the argument. For example, the ``scratch card/card'' entity is linked to the patients of ``receive'' and ``scratch''.
The state is linked to a step on two conditions: the state's argument contains the step's action and predicates, or the state's argument contains the step's action and the state's grandparent~(sub-entity) is linked to the step's arguments. \par

% \subsection{Baseling Approaches}
% We use the LTP 4.0 tool~\cite{che2020n} to do word and sentence segmentation. 
\paragraph{Backbone parsers}We leverage four state-of-the-art pre-trained semantic dependency parsers~\footnote{We use the Biaffine and MFVI implemented in \url{https://github.com/yzhangcs/parser} and the latest official version of LTP and HanLP. All parsers are pre-trained on the same corpus.} as our backbone to parse the sentences:
\begin{itemize}
    \item Biaffine~\cite{dozat2018simpler} uses a multilayer bi-LSTM and biaffine classifiers to train and produce the graph of semantic dependencies;
    \item MFVI~\cite{wang2019second} extends the Biaffine parser by using mean field variational inference to get second-order parsing;
    \item HanLP~\cite{he2020establishing} extends the Biaffine parser by replacing the bi-LSTM encoder with BERT~\cite{devlin2019bert};
    \item LTP~\cite{che2020n} extends the Biaffine parser by replacing the bi-LSTM encoder with the pre-trained Electra model~\cite{clark2019electra}.
    
\end{itemize}
\paragraph{Baseline approaches}Combined with the procedure-first and declaration-first, we get eight baseline approaches in total to benchmark this task. They are named as Binafiine-\khs, MFVI-\khs, LTP-\khs, HanLP-\khs, Binafiine-\kts, MFVI-\kts, LTP-\kts, and HanLP-\kts.

% \paragraph{3) Align the labels.}
% \paragraph{}
% If the sentence is imperative, we assign the user entity to the agent of the core predicate. For example, 

% \subsection{The heuristic framework}
% To automatically extract knowledge described in Sec.~\ref{sec:task_rep}, we divide user instructions into sentences and propose a pipeline framework~(Figure~\ref{fig:framework}):
% \paragraph{1) Sentence segmentation:}The raw user instructions are segmented into sentences via the LTP 4.0 tool~\cite{che2020n}.
% \paragraph{1) Semantic dependency parsing.}We employ the idea of using semantic dependency parsing to get the sentence-level knowledge units and the dependencies. This is based on the previous techniques~\cite{kazeminejad_automatic_2021,brown2022semantic} on \kh not issued by human~(e.g., photosynthesis) and our observations that the knowledge dependency and the semantic dependency of user instructions are somewhat alike in logical form. Specifically, we use a pre-trained semantic dependency parser, e.g., LTP-SDP~\cite{che2020n}, to parse the sentences. If a sentence is imperative, empirically, we can estimate the agent of the core predicate is the user. In a similar manner, we change all ``you'', ``your'' to ``user'' and ``user's'', respectively. Semantic dependency parser treats each single word as a node, but we desire units defined in Sec.~\ref{sec:task_rep}. Thus, 7 In particular, given a predicate, except for its agent, the offsprings of its child is combined to the child to compose a meaningful phrase.
% \paragraph{2) Separate \kh and \kt.}We propose two heuristic strategies~(\kh first and \kt first) to do the separation. The \kh first strategy assume two consecutive user-issued predicates form a \kh boundary, and the rest are \kt. The \kh first strategy assume that if the predicate's agent is an ``EXP'' or not the user, it and its arguments belong to \kt; otherwise, they belong to \kh.
% \paragraph{3) Eliminate leaf nodes:}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=7cm]{figures/framework.png}
%     \caption{The pipeline framework to extract knowledge from user instructions}
%     \label{fig:framework}
% \end{figure}
% \paragraph{3)-1 Fuse \kh.}We fuse two separate \kh boundaries into a new boundary on one condition --- they share at least one predicate and its patients. We treat the larger \kh boundary as the base and traverse it until the first shared predicate. Concatenate the predicates before this predicate to the first predicate of the smaller boundary and concatenate the last predicate of the smaller boundary to the predicates after this predicate. Further, we combine the arguments of the shared predicates. This process continues until there remains only one boundary or the remaining boundaries cannot be inserted to each other any more. The predicate is the action of a step, together with the time, location, and manner, making up a step. The alignment of arguments and semantic labels is listed in Appx.~\ref{sec:align} Table~\ref{tab:alig_kh}.
% \paragraph{3)-2 Fuse \kt.}The rest of the user instructions is \kt. Besides the user entity, we use the overlapping set of agents in \kt and objects in \kh as the primary entity set. If a node is the ``FEAT'' to an entity, then ``[node]entity'' is a sub-entity of the entity. If the sub-entity is the ``FEAT'' to a node, the node is a property to the sub-entity. If a node is the ``LINK-Clas'' to an entity's predicate, we add a ``role'' property to the entity and the node is the value of ``role''. If a node is the ``LINK-Belg'' to an entity's predicate, we add use the node as a property of the entity. The remaining predicates are added to the forth level of \kt according to the entities/sub-entities/properties in the arguments. Note that, the user entity has the first priority. In the same manner with the annotation, sub-entities without any offsprings along with their parents will be removed from \kt.
% The alignment of units in \kt and semantic labels is listed in Appx.~\ref{sec:align} Table~\ref{tab:alig_kt}.

% For the visualization of this pipeline, please refer to Appx.~\ref{sec:pipe}.








==> chapters-old/data-old.tex <==
\section{The \dataname dataset}
\subsection{Definition}
\label{sec:task_rep}
% \paragraph{Definition}
We propose a new benchmark for automated comprehension of user instructions. Specifically, it requires the system to answer the following styles of questions.
\begin{itemize}
    \item Factoid-style questions: asking for the arguments of an action~(the first question in Figure~\ref{fig:style}) or the details of the entities~(``how long will the card be invalid'').
    \item Procedure-style questions: asking for the following steps~(``I have signed in the APP, what's next'') or asking for the missing arguments of a step~(the second question in Figure~\ref{fig:style}).
    \item Inconsistent questions: asking for the reasons that cause the inconsistency with the user instruction~(the third question in Figure~\ref{fig:style}).
\end{itemize}
\par
% To answer these questions, it needs the system to comprehend the procedural information and the declarative information grounding it. Specifically, we define the procedure in the user instructions as a sequence of steps that should be taken by the user. Each step has an action, which consists of a verb~(e.g., ``earn'') and the verb mark~(e.g., ``up to''). The action has arguments~(patient, time, location and manner). Thus, the action can be represented as an n-tuple \{verb|mark, patient, time, location, manner\}, e.g., \{``earn|up to'', ``[\$10] cashback'', ``'', ``'', ``''\}. Further, we define the declaration as a set of entities grounding the procedure. Each entity is a four-layer hierarchical tree --- the root node is entity~(e.g.,``user''); the second layer contains its sub-entities~(e.g., ``[real-name authenticated] user''), ``[] entity'' is used as the default sub-entity of an entity; the third layer contains the properties~(e.g., ``hit rate'') and their values of the sub-entities~(e.g., ``100\%''), ``global property'' is used as the default property of a sub-entity; the forth layer contains states of the properties. Thus, the entire information of a leaf node can be represented as \{entity, sub-entity, property|value, state|value\}, e.g., \{``scratch card'', ``[]scratch card'', ``hit rate|100\%'',``'',``''\}. The state inherits the definition of the step and has an additional cause argument for the action, represented as \{verb|mark, patient, time, location, manner, cause\}. Each procedure has only one user entity. The grounding of the declarative information to the procedural information is annotated as the link from the user entity to the procedure, the links from non-user entities to action arguments~(entity link), and the links from the states to steps~(state link). Note that, the user entity has the highest priority, as it grounds all steps of the procedure. Each entity must be linked to at least one argument. 
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/evidence_new.png}
    \caption{The process to answer the inconsistent questions through the annotation results.}
    \label{fig:reason}
\end{figure*}

\input{tables/question_survey.tex}
\subsection{Annotation}
\label{sec:ann}
We are interested in the Chinese helping documents from an e-commerce company. These documents are written by the marketing staffs for promotions. After pre-processing, we collect a dataset of 1928 user instructions. Each user instruction contains a title and the instructive content, as shown in Figure~\ref{fig:example} (a). \par 
Following \citet{dalvi2018tracking}, we reduce the three styles of questions~(cf., Section \ref{sec:task_rep}) into seven template questions:
\begin{enumerate}[label=\texttt{Q\arabic*}.]
    \item what are the actions in the procedure? 
    \item What are arguments~(patient, time, location and manner) of an action? 
    \item What's the order of the actions?
    \item What are the entities grounding the procedure? 
    \item What are the details~(sub-entity, property, state) of an entity?
    \item Is an entity or sub-entity linked to the argument of an action?
    \item Is a state linked to the step?
\end{enumerate}
Specifically, \texttt{Q1}-\texttt{Q3} are designed for the procedure, \texttt{Q4} and \texttt{Q5} are designed for the declaration, \texttt{Q4} and \texttt{Q5} are designed for the grounding. If the above questions can be answered, the majority of higher-level questions~(factoid-style, procedure-style and inconsistent questions) can also be answered.
The answers for \texttt{Q1} and \texttt{Q4} are text spans~(e.g., ``sign in''), for \texttt{Q3} is an ordered action list~(e.g., [``sign in'', ``tap'', ``pay'', ``receive'', ``scratch'', ``earn'']), for \texttt{Q2} and \texttt{Q5} are n-tuples of text spans~(e.g., \{``APP'',``'',``'',``'' \} of ``sign in''), for \texttt{Q6} and \texttt{Q7} are YES/NO. \par
We randomly select 200 samples and recruit three workers to annotate them according to the template questions\footnote{The annotation is done on the annotation platform of the e-commercial company. We will release the HTML codes for the annotation interface at \url{http://github.com/<anonymized>}.}. An example of annotated user instructions is presented in Figure~\ref{fig:example} (c)---the \textcolor{orange}{left part} is the sequence of steps, each step consists of an action and its arguments~(e.g., manner); the \textcolor{cyan}{right part} contains the set of entities, each entity is a four-layer hierarchical tree; the grounding involves the user entity linked to all steps~(\userlink), the entities linked to the arguments of an action~(\entitylink), and the state linked to a step~(\statelink).
\input{tables/statis}
\paragraph{Discussion:} While it is clear that the annotations can answer the factoid-style and procedure-style questions~\cite{dalvi2018tracking}, we reuse the third question in Figure~\ref{fig:style} to explain how the annotations can support inconsistent questions. Given the question, user instruction and the database, the inference path of the answer on the annotation results is highlighted in black in Figure~\ref{fig:style}. After the inference, the system can obtain one hint that needed to be checked by the system and three hints that needed to be checked by the questioner, as shown in Figure~\ref{fig:reason}. The former hint is accepted only if the system finds that the issued scratch cards have reached the total number. Otherwise, the system response the questioner with clarification questions composed from the latter hints.


\paragraph{Quality control:}An annotated result is accepted only if all three workers agree; otherwise, we invite two experts~(one is from the marketing department, the other is a NLP researcher) to make the final decisions. The experts closely discuss with each other to ensure the results' consistency. 
\paragraph{Data analysis:}Towards a clear picture of the annotated dataset, we list some key statistics in Table~\ref{tab:statistic}. Note that, a document may contain more than one procedure.



% \paragraph{Data Analysis:} 
% In reporting these statistics, we perform word segment using LTP4.0~\cite{che2020n}.

% The answers of these questions require the system to inference on \kt, \kh, and across them by their groundedness, respectively. Noticeably, we design a novel formulation for \texttt{T3}, as shown in Figure~\ref{fig:reason}. On the one hand, if the system find a definite evidence, it responses the user following the traditions. For example, after checking the database, the system find the the user fails to receive scratch card because all cards have been issued, the answer can be ``The scratch cards are out''. On the other hand, if the system cannot find a definite evidence, its response is a confirming table with potential evidences associated with the user. For example, if the scratch cards are sufficient in stock, the system responds the user with the user-related evidences.\par
% Along with the proposed task, we represent the knowledge of user instructions as $K=\{H, T, G\}$, where $H$, $T$, $G$ are the \kh, \kt and the groundedness, respectively. $H$ is a sequence of steps, each step contains an user-issued action and its arguments~(objects, time, location, manner, cause), all arguments can be void. $T$ is a four-level hierarchical tree. The first level contains the root node, the second level contains the entities~(e.g., ``user'') and sub-entities~(e.g., ``[real-name authenticated] user''), the third level contains the properties~(e.g., ``total number'') of entities and the property values~(e.g., ``100000''), and the forth level contains state elements in the same format with the step in \kh. In particular, we use ``[] entity''~(e.g., ``[] user'') to denote the default sub-entity of an entity, ``global property'' to denote the default property of a sub-entity, ``-'' to denote the default value of a property, ``action|mark'' to denote the action~(e.g., ``limit'') and its mark~(e.g., ``passive''). Note that, the user entity has the highest priority, as it dominates all steps in \kh. Each entity in the second level of \kt must be linked to at least one argument in \kh. Only the elements in forth layer can be linked to the step in \kh. Figure~\ref{fig:example} (c) displays an example of this knowledge representation.
% \subsection{Knowledge Representation}

% \subsection{Data Collection \& Annotation}
% We are interested in the Chinese helping documents for promotions from an e-commerce company. The documents are written by the marketing department and are available to custom service staffs. A custom service staff is required to help the custom get involved in promotions successfully following the instructions in the helping documents. After pre-processing, we collect a dataset of 1928 user instructions, whose topics ranges from long-term marketing~(e.g., “get bonus by inviting new users”) to short-term promotions (e.g., holiday promotions). Each user instruction contains a title and the instructive content, as shown in Figure~\ref{fig:example} (a). \par 
% We randomly select 200 samples and recruit three workers to annotate them according to the following steps. 

% \begin{enumerate}[label=(\arabic*)]
%     \item Boundary annotation: The \kh sentences may be interspersed with \kt sentences, for example, ``The total ... 100\%'' in Figure~\ref{fig:example} (a). Besides, a sentence may contain both \kh and \kt. As a result, the first task is annotate the boundaries of \kh. The rest sentences or sub-sentences belong to \kt.
%     \item Boundary Fusion: If a document have multiple boundaries, we ask the workers to fuse the boundaries to form procedures. Note that, the boundaries in a document can form more than one procedure.
%     \item Fine-grained \kh annotation:  After the fusion, the workers annotate the action and arguments of each step.
%     \item Entities extraction: All nouns are extracted from the documents using part-of-speech tool~\cite{che2020n}. The nouns serve as the candidate entities and the nouns with modifiers serve as the candidate sub-entities of \kt. The workers are required to review the candidates and determine final set of entities and sub-entities.
%     \item Fine-grained \kt annotation:  Based on the second level of \kt, the workers are asked to add the offsprings of the \kt tree. Note that, if the sub-entity don't have offsprings, it and its parent entity will be removed from the tree.
%     \item Groundedness annotation: After annotating the details of \kt, the workers are further asked to link entities and states of \kt to \kh.
% \end{enumerate}
% \paragraph{1) Boundary annotation:}The \kh sentences may be interspersed with \kt sentences, for example, ``The total ... 100\%'' in Figure~\ref{fig:example} (a). Besides, a sentence may contain both \kh and \kt. As a result, the first task is annotate the boundaries of \kh. The rest sentences or sub-sentences belong to \kt.
% \paragraph{2) Boundary fusion: }If a document have multiple boundaries, we ask the workers to fuse them to form procedures. Note that, the boundaries in a document can form more than one procedure.
% \paragraph{3) Fine-grained \kh annotation:}After the fusion, the workers annotate the action and arguments of each step.
% \paragraph{4) Entities extraction:}All nouns are extracted from the documents via part-of-speech tagging along with a domain dictionary. The nouns serve as the candidate entities and the nouns with modifiers serve as the candidate sub-entities of \kt. The workers are required to review the candidates and determine final set of entities and sub-entities.
% \paragraph{5) Fine-grained \kt annotation:}Based on the second level of \kt, the workers are asked to add the offsprings of the \kt tree. Note that, if the sub-entity don't have offsprings, it and its parent entity will be removed from the tree.
% \paragraph{6) Groundedness annotation:}After annotating \kt, the workers are asked to link entities and states of \kt to \kh.


    % A toy example of challenging knowledge comprehension: the user has posed a question~(b) that is unexpected to the given user instructions~(a), the system needs to seek out all potential explanations in a ``bottom-up'' manner via inference over \kh, \kt and the groundedness between them.  
    % A user instruction contains all information for ``\chinese{码上返现}~(Earn Cashback with Scan \& Pay)''.  A QA samples: the first question~(\texttt{Q1}) can be answered via the inference about the action states~\cite{dalvi2018tracking}, the second~(\texttt{Q1}) and third question~(\texttt{Q2}) need inference on \kh, \kt and the groundedness between them. (c) The annotated user instruction supporting the knowledge comprehension and complex inference:
    % The \kh is colored in \textcolor{orange}{orange}, the \kt is colored in \textcolor{cyan}{cyan}, the groundedness between them is colored in \textcolor{gray}{gray}, and the inference path is highlighted in black. Best viewed in color.



==> chapters-old/data-v1.tex <==
\subsection{The \dataname dataset}
\begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{figures/q-stat.png}
    \caption{Dataset statistics}
    \label{fig:qstat}
\end{figure}

We are interested in the Chinese helping documents from an e-commerce company. These documents are written by the marketing staffs for promotions. After pre-processing, we collect a dataset of 1928 user instructions. Each user instruction contains a title and the instructive content, as shown in Figure~\ref{fig:example} (a). \par 
Following \citet{dalvi2018tracking}, we reduce the three styles of questions~(cf., Section \ref{sec:task_rep}) into seven template questions:
\begin{enumerate}[label=\texttt{Q\arabic*}.]
    \item what are the actions in the procedure? 
    \item What are arguments~(patient, time, location and manner) of an action? 
    \item What's the order of the actions?
    \item What are the entities grounding the procedure? 
    \item What are the details~(sub-entity, property, state) of an entity?
    \item Is an entity or sub-entity linked to the argument of an action?
    \item Is a state linked to the step?
\end{enumerate}
Specifically, \texttt{Q1}-\texttt{Q3} are designed for the procedure, \texttt{Q4} and \texttt{Q5} are designed for the declaration, \texttt{Q4} and \texttt{Q5} are designed for the grounding. If the above questions can be answered, the majority of higher-level questions~(factoid-style, procedure-style and inconsistent questions) can also be answered.
The answers for \texttt{Q1} and \texttt{Q4} are text spans~(e.g., ``sign in''), for \texttt{Q3} is an ordered action list~(e.g., [``sign in'', ``tap'', ``pay'', ``receive'', ``scratch'', ``earn'']), for \texttt{Q2} and \texttt{Q5} are n-tuples of text spans~(e.g., \{``APP'',``'',``'',``'' \} of ``sign in''), for \texttt{Q6} and \texttt{Q7} are YES/NO. \par
We randomly select 200 samples and recruit three workers to annotate them according to the template questions\footnote{The annotation is done on the annotation platform of the e-commercial company. We will release the HTML codes for the annotation interface at \url{http://github.com/<anonymized>}.}. An example of annotated user instructions is presented in Figure~\ref{fig:example} (c)---the \textcolor{orange}{left part} is the sequence of steps, each step consists of an action and its arguments~(e.g., manner); the \textcolor{cyan}{right part} contains the set of entities, each entity is a four-layer hierarchical tree; the grounding involves the user entity linked to all steps~(\userlink), the entities linked to the arguments of an action~(\entitylink), and the state linked to a step~(\statelink).
\input{tables/statis}
\paragraph{Discussion:} While it is clear that the annotations can answer the factoid-style and procedure-style questions~\cite{dalvi2018tracking}, we reuse the third question in Figure~\ref{fig:style} to explain how the annotations can support inconsistent questions. Given the question, user instruction and the database, the inference path of the answer on the annotation results is highlighted in black in Figure~\ref{fig:style}. After the inference, the system can obtain one hint that needed to be checked by the system and three hints that needed to be checked by the questioner, as shown in Figure~\ref{fig:reason}. The former hint is accepted only if the system finds that the issued scratch cards have reached the total number. Otherwise, the system response the questioner with clarification questions composed from the latter hints.


\paragraph{Quality control:}An annotated result is accepted only if all three workers agree; otherwise, we invite two experts~(one is from the marketing department, the other is a NLP researcher) to make the final decisions. The experts closely discuss with each other to ensure the results' consistency. 
\paragraph{Data analysis:}Towards a clear picture of the annotated dataset, we list some key statistics in Table~\ref{tab:statistic}. Note that, a document may contain more than one procedure.




==> chapters-old/dicussion.tex <==
% future work：道阻且长，行则将至
\subsection{Analysis}
The necessity of mapping user instructions into structured knowledge has been well discussed and experimentally demonstrated in a handful of previous works~\cite{nabizadeh2020myfixit,tandon-etal-2020-dataset,pal2021constructing,bombieri-EtAl:2022:LREC}. 
Based on these discussions and demonstrations, in this section, we are interested in the benefits that can be gained from the integrated comprehension of user instructions and the issues of current study.
\paragraph{Benefits} As we mentioned in Sec.\ref{sec:intro}, the integrated comprehension of user instructions makes it possible to answer factoid-style, procedure-style and inconsistency questions. This is important to achieve human-level machine intelligence, especially the human-level QA bot. In addition to the inference ability on existing user instructions, the integrated comprehension sheds lights on the reasoning and planning of new tasks. Possible applications involve the arrangement of unordered actions, error detection of the draft user instructions, automated composition of user instructions, etc. The system, with the ability to do integrated comprehension, can further be applied in downstream scenarios other than QA. For example, such a system is beneficial to build an intelligent training bot for new staffs of the custom service department via interactive instructions, automatic testing, etc.
\subsection{Issues} In Sec.~\ref{sec:results}, we point out that the cascading errors damage the performance of systems. This issue may be eliminated to design an end-to-end model with large-scale corpus. After a detailed investigation of the failed cases, we report four issues that needed to be further improved. The first issue is co-reference that two separate terms are used to describe the same domain-concept, e.g., ``scratch card'' and ``card'' in Figure~\ref{fig:example} (a). This may lead to the redundancy of entity trees and the missing of entity links. The second issue is the long sentence with more than one action, more than one entity or with both actions and entities. This may lead to the omission of actions or the over-production of useless actions. The third issue is the multi-agent user instructions that need more than one participant to achieve the goal. For example, to attend the promotion of ``Get bonus by inviting your friend'', both the user and the friend are required to issue some actions. To comprehend such user instructions raise new challenges~(e.g., the relation between the user's procedure and the friend's procedure)for the system. The forth issue is the user instruction may be multi-modal. This requires the system align the information in text and images in both factoid-style and procedure-style.
% The above two issues together pose the third issue of 
% \begin{itemize}
%     \item multi-domain and open vocabulary
%     \item Issue of accumulated error.
%     \item Issue of co-reference
%     \item Issue of missing \kh and \kt.
% \end{itemize}




% \paragraph{Future Directions}
% Based on the benefits and issues, we suggest several future directions:
% \begin{itemize}
%     \item KG-enhanced comprehension:
%     \item Multi-agent user instruction comprehension:
%     \item Multi
%     \item Application in real-word scenarios. language-grounding tasks (video instructions,  robots)
% \end{itemize}









==> chapters-old/intro___1225.tex <==
\section{Introduction}
\label{sec:intro}

User manuals, well-designed by experts,
% ~(e.g., technicians or marketing specialists), 
are supposed to be helpful in using products, getting involved in promotions~(as shown in Figure~\ref{fig:manual}),
% de_rijke_question_2005,
or other goals of interest~\cite{chu2017distilling,bombieri2021automatic}. Though instructive, they are seldom read by users because ``\textit{Life is too short to read manuals}''~\cite{8154819}. Towards high user satisfaction, professional customer service representatives~(CSRs) are hired to do the reading and answer questions about the manuals. The machine comprehension of user manuals thus has huge potential, as it would not only reduce labor costs but enable the service ready for customers 24/7. 
% However, it is challenging to get a machine that can understand user manuals as well as a professional.
\par

% \begin{figure}
%     \centering
%     \includegraphics[width=7.5cm]{figures/manual.png}
%     \caption{Example of a user manual with \textcolor{orange}{procedural} and \textcolor{cyan}{declarative} information.}
%     \label{fig:manual}
% \end{figure}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/style.png}
%     \caption{Examples of the three styles of questions about the user manual in Figure~\ref{fig:manual}. To answer these questions, a CSR needs to not only search the arguments of steps or facts but infer along with the steps and the facts binding the steps. Contents related to the answers are highlighted in yellow.
%     }
%     \label{fig:style}
%     \vspace*{-0.6cm}
% \end{figure*}

% Let's take a close look at the user manual for the promotion of ``Earn Cashback with Scan \& Pay'' in Figure~\ref{fig:manual}. It is a standard user manual, with both procedural and declarative information~\cite{smith1984understanding,karreman2005procedural}. The procedural information, colored in orange, describes the steps needs the user to take~(e.g., ``Sign in the App'').  
% The declarative information, colored in cyan, involves facts binding the steps~(e.g., ``The same user can only have up to 10 cards during the promotion period''). \par


However, it is not easy for a machine to understand user manuals like a professional. Current studies have found limitations of factoid-style machine comprehension and
% paid more attention to 
centered on answering procedure-style questions.
% maeta2015framework,nabizadeh2020myfixit,
Despite continuous efforts~\cite{kiddon_mise_2015,vaucher2020automated,goyal2021tracking},
% \textbf
{they usually fail to answer more complex questions
than factoid- and procedure-style ones}.
% The third question in 
Figure~\ref{fig:style} demonstrates an example of the complex question.
% --- the user didn't get the expected reward when participating in the promotion described in Figure~\ref{fig:manual}. 
As this question describes an unexpected case inconsistent with the user manual~(Figure~\ref{fig:manual}), we call it an \textbf{inconsistent question}. 
% This type of question plays a significant part~(approximately a quarter) in real-world e-commercial customer service~(Table~\ref{tab:q_survey}). 
To answer the question, a CSR should carefully read both procedural~(colored in orange) and declarative~(colored in cyan) information
% of the user manual 
and find related clues. 
% Specifically, if 
If the CSR finds the scratch cards have run out after querying the database, she could answer the question directly. Otherwise, she should find more clues by consulting the user.
% about the number of received cards, etc.
Inspired by the CSR, we believe
% The first thing we learn from the CRS is that 
% \textbf
{the integrated understanding of procedural and declarative knowledge can advance the machine comprehension of user manuals}.\par
% A statistical analysis of user questions~(Table~\ref{tab:q_survey}) shows that inconsistent questions play a significant part~(approximately a quarter) in real-world e-commercial customer service.
% \vspace*{-0.05cm}
In this paper, we wish the machine comprehension of user manuals goes a step closer to CSRs in the e-commercial scenario.
% Note that, w
We don't expect the machine to replace CSRs at present. Instead, we hope the machine can at least be an assistant to save the labor costs of information searching by suggesting/highlighting answers or clues to the answers.
% ~(e.g., highlighting contents in Figure~\ref{fig:style}). 
There are two minimum requirements to make CSRs use the machine's suggestions --- 1) the machine is \textbf{robust} about various questions to provide trustable suggestions for CSRs; 2) the machine is \textbf{interpretable} about its suggestions~(answers or clues) to provide more flexibility for CSRs. \par
% To concrete the study of such machine comprehension systems, 

To this end, we propose the \textbf{\kh \& \kt benchmark}. It requires the machine to fully understand a user manual and find the answers or clues for factoid-style, procedure-style, and inconsistent questions about the manual. We name this benchmark after Gilbert Ryle's thought about the
% ~\cite{ryle2009concept,bengson2011knowing,pavese_knowledge_2021}
intelligence~\cite{ryle2009concept}\footnote{Gilbert Ryle thought that the possession of \kh~(i.e., procedural knowledge) and \kt~(i.e., declarative knowledge) is ``a mark of intelligence''.}. To establish the benchmark, we collect a corpus~(\dataname) of 10000 user manuals~(i.e.,  \underline{O}nline \underline{H}elp d\underline{O}cuments) that are frequently visited by customer service representatives from an e-commercial platform. Each manual is along with one or more unanswered FAQs. 
Based on \dataname, we annotated two datasets
% ~(\dataname-E and \dataname-I) 
to perform extrinsic and intrinsic evaluations for the machine comprehension of user manuals, respectively. First, we randomly sample 2000 questions and hand annotate their answers.
% , i.e., \dataname-E. 
We build a \underline{H}euristic and inherently interpretable baseline to understand \underline{U}ser \underline{M}anuals based on semantic parsing, named HUM. It performs impressively better and more robustly than off-the-shelf methods, revealing the big advantages made by the joint parsing of procedural information, declarative information, and how declarative information binds the procedural information.
Second, we randomly sample 200 user manuals and annotate the answers to seed questions about each manual.
% , i.e., \dataname-I. 
% In this way, 
We then use the answers to parse each manual into its structured representation, a heterogeneous graph with two types of nodes and three groups of relations. The representation enables machine inference for higher-level questions and thus allows us to estimate the upper bound of machine comprehension from the omniscient view.
% , estimating the upper bound to answer various questions about a user manual. 
% The first dataset consists of 2000 randomly sampled FAQs and their hand-annotated answer spans    
% We further annotate two datasets based on sampled FAQs and seed questions for extrinsic and intrinsic evaluations, respectively.  
% We annotate the answers for a subset of questions to
% We randomly sample 2000 questions and hand annotate their answers for developing and testing. 
% % Each answer involves one or more text spans in the user manual. 
% This dataset enables us to 
% extrinsically investigate the machine comprehension of different user manuals.
% with real-world answers. 
% Inspired by the annotation of state changing in procedure~\cite{dalvi2018tracking}, 
% We build a \underline{H}euristic and inherently interpretable baseline to understand \underline{U}ser \underline{M}anuals based on semantic parsing, named HUM. The HUM model performs impressively better and more robustly than off-the-shelf methods, because of its joint parsing of procedural information, declarative information, and how declarative information binds the procedural information.
% This baseline is inherently robust, as it can jointly parse procedural information, declarative information, and how declarative information binds the procedural information. It is also interpretable because of its dependency structure among the units.
% We also conduct an intrinsic annotation on a subset of user manuals, inspired by \citet{dalvi2018tracking}.
% . 
% Each manual is presented as a heterogeneous graph based on seven seed questions.
% This dataset allows us to estimate the machine's intelligence to answer various questions about the same user manual.
% Inspired by the annotation of state changing in procedure~\cite{dalvi2018tracking}, we represent a user manual as a sequence of steps, a set of facts, and the bindingness. 
% we believe exploring unsupervised resolutions is the desired choice for the machine comprehension of user manuals in smart customer service.
% Considering the fact that the user manuals in e-commercial scenarios are continually updating and increasing, we believe exploring unsupervised resolutions 
% We then build a heuristic method based on semantic parsing to gain robustness and interpretation simultaneously.
% Each manual is constructed as a heterogeneous graph based on seven seed questions.
Through a systematic comparison of eight variants of HUM and the indicative upper bound, we find that there remains a large margin for the machine to get human-level comprehension of user manuals
and more effort is demanded. Carefully analyzing the failed cases of machines, we point out the future challenges lying in co-reference, accumulative errors, and discourse parsing beyond sentences. As a step further, we also pose the potential studies boosted by the proposed benchmark and the annotated datasets\footnote{The \dataname corpus, baseline approaches, and evaluation results will be made available at \url{http://github.com/<anonymized>}.}. 
\par

In summary, we highlight our work in three points: (1) We propose the novel \kh \& \kt benchmark. It opens a chance to study the machine comprehension of user manuals in a more challenging setting, which requires the machine to answer various user questions, including complex ones. (2) We elaborately establish the benchmark with a corpus of real-world user manuals, two hand-annotated testing sets, and a robust and inherently interpretable baseline. This further enables the extrinsic and intrinsic evaluations of machine comprehension in actually observed and omniscient scenarios, respectively. (3) Based on the empirical results, we call attention to the integrated comprehension of user manuals and present the challenges for the machine to gain human-level comprehension. We wish our work can shine a light on the more advanced machine comprehension of user manuals in smart custom services or a broader range of applications.


==> chapters-old/intro___v2.tex <==
\section{Introduction}
\label{sec:intro}
User manuals, well-designed by experts, are supposed to be helpful in using products, getting involved in promotions, or other goals of interest~\cite{ryle2009concept,chu2017distilling,bombieri2021automatic}. Though instructive, they are seldom read by users because ``\textit{Life is too short to read manuals}''~\cite{8154819}. Towards high user satisfaction, professional customer service representatives~(CSRs) are hired to do the reading and answer user questions about the manuals. The machine comprehension of user manuals thus has huge potential, as it would not only reduce labor costs but enable the service ready for customers 24/7. 
\par
\begin{figure}[t]
    \centering
    \includegraphics[width=6.8cm]{figures/style.png}
    \caption{A user manual and three question-answering cases about it
    % . Key phrases of questions and answers are highlighted in bold, colors, and underlines.
    }
    \label{fig:style}
\end{figure}
Before going deep into such machine comprehension, let's see how a CSR approaches various questions given the user manual in Figure~\ref{fig:style}. Specifically, she can answer Q1 by looking up the arguments of facts, i.e., the value (\colorbox{Purple!30}{100\%}) of \textcolor{Purple}{the hit rate}. For Q2, she reasons about the procedure and finds the answer~(\colorbox{Green!30}{on the payment page}) from the step before \textcolor{Green}{scratching the card}. The hardest question is Q3, which poses a case~(\textcolor{BrickRed}{haven't} \textcolor{Cerulean}{gotten the scratch card}) \textbf{inconsistent} with the user manual. To answer it, she needs to find both factoid and procedural clues to the question and provide proper responses, i.e., the answer~(A1) or clarifying questions~(A2-A4). Intuitively, the most straightforward solution for Q3 is to check every step and fact with the user, yet heavily damage the user satisfaction. Aligned with the CSR, the practical machine comprehension model must be able to identify the type of questions and draw proper inference across the user manual, for example, only infer about the arguments for Q1.\par
% Hence, to achieve practical machine comprehension for customer service, a model must be able to reason not only about the procedure but the facts binding the steps.
Currently, the machine comprehension for factoid-style questions~(e.g., Q1) has built a splendid library of studies, running from one-span answers to multiple-span answers~\cite{rajpurkar2016squad,zhu2020question}. More recent studies~\cite{tandon-etal-2020-dataset,goyal2021tracking,zhang2021knowledge} have found the weakness of factoid-style comprehension on procedure-style questions. However, these studies are centered mainly on questions about the states of entities that can be answered by single spans. They have trouble answering more complex procedure-style questions with multiple-span answers or the dynamic arguments of actions~(e.g., Q2), let alone inconsistent questions like Q3. Moreover, we notice that existing datasets and models are designed for single types of questions. This doesn't meet the real-world customer service scenario where both consistent~(i.e., factoid-style and procedure-style) and inconsistent questions are involved~(cf., Table 1).\par



% Moreover, we find that inconsistent questions~(e.g., Q3), nearly one-quarter of real-world user questions~(cf., Table 1), have been virtually overlooked by the existing research.  
% All of these motivate us to take a step forward and study the machine comprehension of user manuals in a more natural but challenging setting, which involves factoid-style, procedure-style, and inconsistent questions.


% Current research is focused on either factoid-style questions~\cite{rajpurkar2016squad,jiang2020recipe,nabizadeh2020myfixit} or procedure-style questions~\cite{vaucher2020automated,goyal2021tracking}

% However, current research is largely focused on user questions consistent with the user manual, especially the factoid ones~\cite{rajpurkar2016squad,jiang2020recipe,nabizadeh2020myfixit}. Although more recent studies~\cite{vaucher2020automated,goyal2021tracking} have concerned procedure-style comprehension, they are only centered on questions about the states of entities. As such, they have trouble answering questions about other components like actions in the procedure~(e.g., Q2). 

% the integrated comprehension of procedure knowledge and factoid knowledge.
% \par

% reason not only about the procedure but the facts~(e.g., \colorbox{Cerulean!30}{the total number of scratch cards is 10000})~binding the steps. Hence, to achieve machine comprehension of user manuals for customer service, a model is required to 1


% To answer Q3, tougher than Q1 and Q2, she reasons not only about the procedure but the facts binding the steps.



% To realize such machine comprehension, a model needs to fully grasp the user manual and identify answers to various questions about it. 
% Hence, it requires 
% Current studies are mainly focused on questions that are consistent with the user manuals.
% Based on the user manual in Figure~\ref{fig:style}, we present three types of user questions. Massive efforts have been made for the factoid-style question
% To answer the factoid-style question~(Q1), the CSR needs to look up the arguments of facts, such as the value (\colorbox{Purple!30}{100\%}) of \textcolor{Purple}{the hit rate}. To answer the procedure-style question~(Q2), the CSR needs to reason about the steps, e.g., find the location~(\colorbox{Green!30}{on the payment page}) from the previous step of \textcolor{Green}{scratch the card}. 

% Q1 is a factoid-style question that requires the CSR to look up the arguments of facts, e.g., query the value (\colorbox{Purple!30}{100\%}) of \textcolor{Purple}{the hit rate}. Q2 is a procedural-style question that requires the CSR to reason about the steps, e.g., find he location~(\colorbox{Green!30}{on the payment page}) from the previous step of \textcolor{Green}{scratch the card}.
% However, current studies are mainly focused on questions that are consistent with the user manual, namely, factoid-style and procedure-style questions as demonstrated in Figure~\ref{fig:style}. Specifically, 



% Based on the user manual in Figure~\ref{fig:style}, we present three types of user questions.
% Fortunately, factoid-style questions~(Q1) have been well-studied 



% However, current studies are mainly focused on user questions that are consistent with the user manual. Specifically, they have 
% Based on the user manual in Figure~\ref{fig:style}, we present three types of user questions. Q1 is a factoid-style question that requires the CSR to look up the arguments of facts, e.g., query the value (\colorbox{Purple!30}{100\%}) of \textcolor{Purple}{the hit rate}. Q2 is a procedural-style question that requires the CSR to reason about the steps, e.g., find he location~(\colorbox{Green!30}{on the payment page}) from the previous step of \textcolor{Green}{scratch the card}.
% Let's look at the customer service scenarios demonstrated in Figure~\ref{fig:style}. To answer Q1, the CSR needs to look up the arguments of facts --- the \colorbox{Purple!30}{value} of \textcolor{Purple}{the hit rate}.
% , i.e., factoid-style comprehension. 
% To answer Q2, the CSR needs to reason about the steps --- find the location~(\colorbox{Green!30}{on the payment page}) from the previous step of \textcolor{Green}{scratch the card}. 
% Tougher than Q1 and Q2, Q3 poses a case~(\textcolor{BrickRed}{haven't} \textcolor{Cerulean}{gotten the scratch card}) that is inconsistent with the user manual. To answer it, tthe CSR needs to reason not only about the steps but the facts binding the steps.
% \par

% To concrete the study, 
To overcome these limitations, we move to a more natural but challenging setting and propose the \textbf{\kh \& \kt} task\footnote{We name it after Gilbert Ryle's thought that the possession of \kh~(i.e., procedural knowledge) and \kt~(i.e., factoid knowledge) is ``a mark of intelligence''~\cite{ryle2009concept}.} --- given a user manual, the model is required to answer factoid-style, procedure-style or inconsistent 
questions about it. This task can be reduced to two fundamental challenges: (\texttt{I}) \textbf{how to extract actions~(entities) and their arguments from the user manual}, (\texttt{II}) \textbf{what is the relation between an action and an entity~(two actions or two entities)}. We resolve these challenges by introducing a structured representation for both questions and user manuals. The representation enables unified inference about various types of questions in the same graph, as shown in Figure~\ref{fig:rep}. We then design a \underline{H}euristic method~(HUM) to map \underline{U}ser \underline{M}anuals into the proposed representations. It is based on pre-trained tools and several efficient rules so that it can further contribute to lowering training costs and improving scalability, which are vital for constantly refreshing industry scenarios. Towards automated evaluation, we collect a testing set~(\dataname) of 2000 \underline{O}nline \underline{H}elp d\underline{O}cuments
from an e-commerce platform. Each manual includes a real-world FAQ and its ground truth answer spans annotated by humans\footnote{Inspired by \citet{rajpurkar2016squad}, we also offer a complementary dataset with 8000 user manuals. Each manual has an unanswered FAQ for related research purposes like self-supervised learning, question generation, etc.}. The proposed method performs impressively better and more robustly than off-the-shelf ones, revealing the big advantages made by the unified inference of actions and entities. To further investigate the remaining challenges and the potential of HUM, we compare its variants with the human upper bound for mapping user manuals into structured representations on 200 user manuals from \dataname. The results show big room for designing better models to get human-level comprehension of user manuals. Specifically, it requires more effort on the co-reference issue, accumulative errors, discourse parsing beyond sentences, etc. We expect our work will contribute to the deep comprehension of user manuals and inspire future research on smart customer service. We summarize our contributions in three points:
\begin{itemize}
    \item We propose the \kh \& \kt task and take the first step to study machine comprehension of user manuals in a more natural but challenging setting, which consists of factoid-style, procedure-style, and inconsistent questions.
    \item We design a structured representation for user questions and manuals coupled with an efficient method~(HUM) that can automatically construct such representation.
    % We propose the \kh \& \kt benchmark requiring the model to answer various questions about user manuals. It is well-armed with a real-world corpus, dense annotations, a competitive baseline, and systematic evaluations. 
    \item The experiment on real-world FAQs reveals the superiority of HUM made by unified inference. Further evaluations about the structured representations point out the significant challenges toward human-level comprehension. 
\end{itemize}
\begin{table*}[t]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{c|c|m{15cm}}
    \hline
      \textbf{Term} &\textbf{Category} & \textbf{Explanation} \\
      \hline
     Action & node & the action of a step performed by the user, presented as a verb, e.g., ``pay''.\\
        \hline
    Entity & node & the unique concepts related to the user manual, e.g., ``scratch card''. Each user manual has a user Entity by default.\\
    \hline
 Action-ARG& argument& the modifier~(\textcolor{orange}{MOD}), time~(\textcolor{orange}{TIME}), location~(\textcolor{orange}{LOC}), manner~(\textcolor{orange}{MANN}), and cause~(\textcolor{orange}{CAUSE}) arguments associated with an Action node. \\
    \hline
    Entity-ARG& argument& the arguments associated with an Entity node --- footnote argument~(\textcolor{NavyBlue}{FN}), offering more details of the entity; attribute argument~(\textcolor{NavyBlue}{ATT}), describing a specific aspect of the entity~(e.g., the hit rate of the scratch card); state argument~(\textcolor{NavyBlue}{STATE}), describing the changeable states of the entity~(e.g., the ``have'' state of the same user). They are derived from the facts binding the steps.\\
    \hline
    ARG-ARG& argument& the arguments associated with an Entity-ARG. The arguments of \textcolor{NavyBlue}{ATT} are the same as Entity-ARG and the arguments of \textcolor{NavyBlue}{STATE} is the same as Action-ARG.\\
        \hline
    
    NEXT & relation & the directed edge between two Action nodes, indicating the end action is the next step of the start one. It determines the order of the actions performed by the user.\\
    \hline
    AGENT&relation& the directed edge from the user Entity node to an Action node, indicating the action is performed by the user.
    % , e.g., the edge from ``user'' to ``pay''.
    \\
    \hline
    PAT& relation& the directed edge from an Action node to an Entity node, indicating the action is performed on the entity.\\
    \hline
    SUB& relation& the directed edge between two Entity nodes, indicating the start entity is a sub-entity of the end one.\\
    \hline
    PATA & relation& the directed edge from a \textcolor{NavyBlue}{STATE} to an Entity node, indicating the entity undergoes the effect caused by the changing of \textcolor{NavyBlue}{STATE}. Note that, the user dominates the whole user manual so that the user Entity cannot be the target of any \textcolor{NavyBlue}{STATE}.\\
    \hline
    \end{tabular}
    }
    \caption{Explanations of nodes, relations, and arguments in the structured representation}
    \label{tab:kg}
\end{table*}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/rep.png}
    \caption{Screenshot of the graph obtained from the user manual and the graphs obtained from Q1, Q2, and Q3}
    \label{fig:rep}
\end{figure*}

% We then design an efficient baseline
% We also design an efficient baseline to automatically map user manuals into structured graphs, which describe the details of actions and facts in addition to their relations.




% It poses two fundamental challenges: what are the details of the steps and facts in 
% Specifically, the model needs to tell us the details of the actions and facts in addition to the relations among them. 
% Towards automated evaluation,
% To establish the benchmark, 

% We also design an efficient baseline to automatically map user manuals into structured graphs, which describe the details of actions and facts in addition to their relations.

% To automatically map user manuals into structured graphs, we also design a \underline{H}euristic baseline to comprehend \underline{U}ser \underline{M}anuals based on semantic parsing, named HUM. 
% To figure out the potential of machine comprehension, 

% and 
% build a subset, involving 200 user manuals from \dataname-\texttt{I}. 
% The annotations of each manual, as shown in Figure 2, enable explicit inference about various questions. 


% and annotate a dataset~(\dataname) of user manuals with 2000 FAQs and answer pairs. The user manuals are \underline{O}nline \underline{H}elp d\underline{O}cuments from an e-commerce platform. We then hire CSRs to annotate the answer spans for each questions ,m.lk.
% Each manual is along with one or more unanswered FAQs. In totalWe obtain 2000 FAQs in total
% 2000 user manuals
% , which are \underline{O}nline \underline{H}elp d\underline{O}cuments frequently visited by CSRs from an e-commercial platform. 
% Each manual is along with one or more unanswered FAQs. Based on \dataname, we construct a testing set~(\dataname-\texttt{I}) by annotating the ground truth answers for 2000 randomly sampled questions.



% , are need. As a step further, we also pose the potential studies boosted by the proposed benchmark and the annotated datasets\footnote{The \dataname corpus, baseline approaches, and evaluation results will be made available at \url{http://github.com/<anonymized>}.}. 


% two testing sets and systematically study the machine comprehension of user manuals. 

% We build a \underline{H}euristic and inherently interpretable baseline to understand \underline{U}ser \underline{M}anuals based on semantic parsing, named HUM. It performs impressively better and more robustly than off-the-shelf methods, revealing the big advantages made by the joint parsing of procedural information, declarative information, and how declarative information binds the procedural information.
% Second, we randomly sample 200 user manuals and annotate the answers to seed questions about each manual.

% in user manuals.


% study the machine comprehension of user manuals in a more challenging scenario involving Q1, Q2 and Q3
% --- the model is required to automatically comprehend a user manual and find the answers to various questions~(i.e., factoid-style, procedure-style and inconsistent questions) about it.\par

% This is because they lack an integrated understanding of procedural and declarative knowledge in user manuals and thus fail to reason across steps and facts.\par
% As a step forward, we wish to study the machine comprehension of user manuals in a more challenging scenario --- the model is required to automatically comprehend a user manual and find the answers to various questions~(i.e., factoid-style, procedure-style and inconsistent questions) about it. To this end, 

% To this end, we propose the \textbf{\kh \& \kt benchmark}. It requires the machine to fully understand a user manual and find the answers or clues for factoid-style, procedure-style, and inconsistent questions about the manual. We name this benchmark after Gilbert Ryle's thought about the
% % ~\cite{ryle2009concept,bengson2011knowing,pavese_knowledge_2021}
% intelligence~\cite{ryle2009concept}\footnote{Gilbert Ryle thought that the possession of \kh~(i.e., procedural knowledge) and \kt~(i.e., declarative knowledge) is ``a mark of intelligence''.}. 
 
% Based on \dataname, we annotated two datasets
% % ~(\dataname-E and \dataname-I) 
% to perform extrinsic and intrinsic evaluations for the machine comprehension of user manuals, respectively. First, we randomly sample 2000 questions and hand annotate their answers.
% , i.e., \dataname-E. 

% , i.e., \dataname-I. 
% In this way, 
% We then use the answers to parse each manual into its structured representation, a heterogeneous graph with two types of nodes and three groups of relations. The representation enables machine inference for higher-level questions and thus allows us to estimate the upper bound of machine comprehension from the omniscient view.
% , estimating the upper bound to answer various questions about a user manual. 
% The first dataset consists of 2000 randomly sampled FAQs and their hand-annotated answer spans    
% We further annotate two datasets based on sampled FAQs and seed questions for extrinsic and intrinsic evaluations, respectively.  
% We annotate the answers for a subset of questions to
% We randomly sample 2000 questions and hand annotate their answers for developing and testing. 
% % Each answer involves one or more text spans in the user manual. 
% This dataset enables us to 
% extrinsically investigate the machine comprehension of different user manuals.
% with real-world answers. 
% Inspired by the annotation of state changing in procedure~\cite{dalvi2018tracking}, 
% We build a \underline{H}euristic and inherently interpretable baseline to understand \underline{U}ser \underline{M}anuals based on semantic parsing, named HUM. The HUM model performs impressively better and more robustly than off-the-shelf methods, because of its joint parsing of procedural information, declarative information, and how declarative information binds the procedural information.
% This baseline is inherently robust, as it can jointly parse procedural information, declarative information, and how declarative information binds the procedural information. It is also interpretable because of its dependency structure among the units.
% We also conduct an intrinsic annotation on a subset of user manuals, inspired by \citet{dalvi2018tracking}.
% . 
% Each manual is presented as a heterogeneous graph based on seven seed questions.
% This dataset allows us to estimate the machine's intelligence to answer various questions about the same user manual.
% Inspired by the annotation of state changing in procedure~\cite{dalvi2018tracking}, we represent a user manual as a sequence of steps, a set of facts, and the bindingness. 
% we believe exploring unsupervised resolutions is the desired choice for the machine comprehension of user manuals in smart customer service.
% Considering the fact that the user manuals in e-commercial scenarios are continually updating and increasing, we believe exploring unsupervised resolutions 
% We then build a heuristic method based on semantic parsing to gain robustness and interpretation simultaneously.
% Each manual is constructed as a heterogeneous graph based on seven seed questions.
% Through a systematic comparison of eight variants of HUM and the indicative upper bound, we find that there remains a large margin for the machine to get human-level comprehension of user manuals
% and more effort is demanded. Carefully analyzing the failed cases of machines, we point out the future challenges lying in co-reference, accumulative errors, and discourse parsing beyond sentences. As a step further, we also pose the potential studies boosted by the proposed benchmark and the annotated datasets\footnote{The \dataname corpus, baseline approaches, and evaluation results will be made available at \url{http://github.com/<anonymized>}.}. 
% \par

% In summary, we highlight our work in three points: (1) We propose the novel \kh \& \kt benchmark. It opens a chance to study the machine comprehension of user manuals in a more challenging setting, which requires the machine to answer various user questions, including complex ones. (2) We elaborately establish the benchmark with a corpus of real-world user manuals, two hand-annotated testing sets, and a robust and inherently interpretable baseline. This further enables the extrinsic and intrinsic evaluations of machine comprehension in actually observed and omniscient scenarios, respectively. (3) Based on the empirical results, we call attention to the integrated comprehension of user manuals and present the challenges for the machine to gain human-level comprehension. We wish our work can shine a light on the more advanced machine comprehension of user manuals in smart custom services or a broader range of applications.




==> chapters-old/intro_v1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=7cm]{figures/style_new.png}
    \caption{Examples of the factoid-style, procedure-style and inconsistent questions and their answers.}
    \label{fig:style}
\end{figure}


\section{Introduction}
\label{sec:intro}
% \epigraph{The possession of \kh and \kt is ``a mark of intelligence''.}{\textit{GilBert Ryle \\ The Concept of Mind}}
User manuals are created by experts~(e.g., technicians or marketing specialists) and are supposed to be helpful in using products, getting involved in promotions, or other goals of interest~\cite{de_rijke_question_2005,chu2017distilling,bombieri2021automatic}. Although informative and instructive, these well-designed user manuals are seldom read by end-users because ``\textit{Life is too short to read manuals}''~\cite{8154819}. Towards high-quality customer experience, professionals are hired to completely understand the user manuals and answer various user questions about it. The machine comprehension of user manuals thus has huge potential, as it would not only reduce labor costs but enable the service to be ready for customers 24/7. However, it is very challenging to get a machine that can understand user manuals as well as a human staff.\par

Let's take a close look at the user manual for the promotion of ``Earn Cashback with Scan \& Pay'' in Figure~\ref{fig:style} (a). It is a standard user manual, with both procedural and declarative information~\cite{smith1984understanding,karreman2005procedural}. The procedural information, colored in orange, describes the steps needs the user to take~(e.g., ``Sign in the App''). 
% for the promotion.
% ~(participate in the promotion of ``Earn Cashback with Scan \& Pay''). 
The declarative information, colored in cyan, involves facts grounding the steps~(e.g., ``The same user can only have up to 10 cards during the promotion period''). \par

Current studies have found the limitations of factoid-style machine comprehension and paid more attention to answering procedure-style questions~\cite{dalvi2018tracking}. Despite continuous advances~\cite{kiddon_mise_2015,maeta2015framework,vaucher2020automated,nabizadeh2020myfixit,kuniyoshi2020annotating,goyal2021tracking}, they have trouble answering more complex questions
than factoid-style and procedure-style questions.
% that need reasoning about not only the procedure but the declarative information grounding it. 
The third question in Figure~\ref{fig:style} demonstrates an example --- the user didn't get the expected reward when participating the promotion. As this question describe an unexpected case not consistent with the user manual, we call this type of questions as inconsistent questions.
% This requirement meets Gilbert Ryle's thought that the possession of \kh~(i.e., procedural information) and \kt~(i.e., declarative information) is ``a mark of intelligence''~\cite{ryle2009concept,bengson2011knowing,pavese_knowledge_2021}. 

% This requires the online platform to hire custom services 
% Although user manuals are written to help users in using products, getting involved in promotions, or other goals of interest, they are not seldom read by people.
% User manuals, while informative and instructive, suffer from over-features
% User instructions, created by experts~(e.g., technicians or marketing staff), play a big part in online platforms. 
% It is a document created by experts~(e.g., technicians or marketing staff) and offered to customer service and end-users~\cite{perelman1996mayfield}. The document provides procedural and declarative information that helps in using products, getting involved in promotions, or other goals of interest~\cite{smith1984understanding,karreman2005procedural}. The automated comprehension of user instructions will benefit a broad range of downstream applications, such as goal-oriented searching~\cite{zook1989effects,yang2015leveraging,chu2017distilling}, question answering~(QA) beyond facts~\cite{de_rijke_question_2005,das2018building,tandon-etal-2020-dataset,pal2021constructing}, language-grounded executable tasks~\cite{costa2017evaluation,bombieri2021automatic}, etc. 






% Specifically, the user needs to 

% The orange sentences are the procedural information that consist of 

% The procedural information contains user actions to reach a goal of interest. the orange sentences are the procedural information to participate in the promotion of ``Earn Cashback with Scan \& Pay'', ``sign in'', ``tap'', etc., are actions that should be taken by the users. The declarative information involves facts grounding the procedure ~(e.g., ``The scratch card will be invalid in one hour once received''). The user can successfully participate in the promotion by carrying out the actions following the right order of the procedure and paying attention to the declarative information. 
% This meets Gilbert Ryle's thought that the possession of \kh~(i.e., procedural knowledge) and \kt~(i.e., declarative knowledge) is ``a mark of intelligence''~\cite{ryle2009concept,bengson2011knowing,pavese_knowledge_2021}. In keeping with Ryle's thought, we believe the integrated comprehension of procedural information and declarative information can significantly advance the system's intelligence in handling user instructions.\par





% Beyond doubt, the user instruction is widespread infiltrating in our everyday life and directly contributes to user satisfaction~\cite{gemoets1990effect,ummelen2022procedural}.
% It can be created by a technician or a marketing staff and acts as an integral part of every product and commercial activity~\cite{renaud2019product,gok2019effect}. The automated comprehension of such user instructions has a board range of downstream applications, such as task-oriented searching~\cite{zook1989effects,yang2015leveraging,chu2017distilling}, question answering~(QA) beyond facts~\cite{de_rijke_question_2005,das2018building,tandon-etal-2020-dataset,pal2021constructing}, language-grounded executable tasks~\cite{costa2017evaluation,bombieri2021automatic}, etc.\par
% 
% Studies~\cite{smith1984understanding,karreman2005procedural} show that a user instruction consists of both procedural and declarative information. The procedural information contains user actions to reach a goal of interest. Take the user instructions in Figure~\ref{fig:style} as an example, the orange sentences are the procedural information to participate in the promotion of ``Earn Cashback with Scan \& Pay'', ``sign in'', ``tap'', etc., are actions that should be taken by the users. The declarative information involves facts grounding the procedure ~(e.g., ``The scratch card will be invalid in one hour once received''). The user can successfully participate in the promotion by carrying out the actions following the right order of the procedure and paying attention to the declarative information. This meets Gilbert Ryle's thought that the possession of \kh~(i.e., procedural knowledge) and \kt~(i.e., declarative knowledge) is ``a mark of intelligence''~\cite{ryle2009concept,bengson2011knowing,pavese_knowledge_2021}. In keeping with Ryle's thought, we believe the integrated comprehension of procedural information and declarative information can significantly advance the system's intelligence in handling user instructions.\par
% A good customer service representative is required to answer any user questions about this manual by searching about the facts, inferring along with the steps, and reasoning about both steps and the facts grounding these steps, as shown in Figure~\ref{fig:style} (b). 
% In keeping with this, we believe the integrated comprehension of procedural and declarative information can significantly advance the machine's intelligence to correctly answer various questions about user manuals.\par

% are still far from enough to human-level comprehension. One of the main reasons is they overlook the grounding of the declarative information on the procedural information.
% To facilitate the automatic evaluations, they have reduced the machine comprehension to the predictions of domain-specific entities~(e.g., the tool entities in repair manuals~\cite{nabizadeh2020myfixit}), changing states of entities~(e.g., the changing power state of the printer~\cite{goyal2021tracking}), actions and its arguments (e.g., the operations and its time condition in scientific experiments~\cite{kuniyoshi2020annotating}), and the order of the actions~\cite{kiddon_mise_2015,maeta2015framework,vaucher2020automated}. 
% Thus, they are largely devoted to the comprehension of procedures. They aim to answer the factoid-style  questions~(the first question in Figure~\ref{fig:style}) and procedure-style questions~(the second question in Figure~\ref{fig:style}). 
% Towards more precisely conduct automatic evaluations, 
% Despite continuous advances, current studies of user instructions are still far from enough to human-level comprehension. One of the main reasons is they overlook the grounding of the declarative information on the procedural information. A direct issue caused by this overlook is that the system has less capability to deal with inconsistent questions (i.e., the questions that user raises when coming across with unexpected cases from the instruction).
%heavily limits the system's ability to deal with questions that have cases not consistent with the user instruction~(inconsistent questions). 

% of complex questions. 
% To answer it, the system needs to grasp an integrated comprehension of the user instruction --- not only the comprehension of procedural information but the declarative information grounding it. In general, the frequency of inconsistent questions is much more than the other two styles. This is because the custom can quickly get the answers of these questions by glancing the helping document\footnote{In fact, through our investigation of the custom service logs from an e-commerce company, more than 90\% questions are inconsistent questions.}.
\par
To break the limitations, we propose a challenging benchmark for user instruction comprehension: given a user instruction, the system is required to answer factoid-style, procedure-style and inconsistent questions. As shown in Figure~\ref{fig:style}, the answers for the former two types of questions are spans from the user instructions, the answers for inconsistent questions could be clarification questions if the system cannot find a definite answer. Inspired by \citet{dalvi2018tracking}, we reduce the three styles of question into seven template questions. The assumption behind is that if the system can correctly answer the template questions, the majority of higher-level questions can also be answered~(cf., Sec.~\ref{sec:ann}). In this way, we create the \dataname corpus with 1928 Chinese \underline{He}lping \underline{Do}cuments from an e-commerce company and densely annotate 200 documents based on the template questions for testing. Further, we design eight baseline approaches to produce the answers of the template questions. Interesting, all approaches get consistent low performances even on the template questions. This indicates that the integrated comprehension of user instructions is challenging and more efforts are demanded. Further, through a deep look at the dataset and failed cases, we pose the benefits of this new task, the current issues and possible directions for future work. The \dataname corpus, baseline approaches and evaluation results will be made available at \url{http://github.com/<anonymized>}.\par
In summary, our work has three contributions:
  \begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/example_inconsistent.png}
    \caption{Illustration of a user instruction~(a), an inconsistent question~(b), and the annotated user instruction~(c), whose \textcolor{orange}{left part} is the sequence of steps, \textcolor{cyan}{right part} contains the set of entities, and \userlink, \entitylink, and \statelink are the 
    the grounding from the declaration to the procedure.
    }
    % \vspace{-0.6cm}
    \label{fig:example}
\end{figure*}
\begin{itemize}
    \item We propose a new benchmark for  user instruction comprehension. Given a user instruction, it requires the system to answer factoid-style, procedure-style and inconsistency questions.
    \item The benchmark involves a new corpus~(\dataname) of helping documents equipped with a hand-annotated test set, eight baseline approaches and an automated evaluation method.
    \item Experimental results reveal the significant challenges of this new task. By human analysis, we further point out the benefits of this study, key issues and the possible directions.
\end{itemize}
%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.88\textwidth]{figures/example.png}
%     \caption{Illustration of the user instruction for ``\chinese{使用手机号注册支付宝国际账户}~(Registration of Alipay International Account with Phone Number)''~(the upper block). The lower block shows how \kh and \kt are grounded~(blue lines), in addition to the constructions of complex knowledge~(left is the \kh and right is the \kt).}
%     \label{fig:example}
% \end{figure}
                          















==> chapters-old/old.tex <==
Among the mainstream knowledge extraction methods, entity extraction, also known as named entities recognition (NER), is a basic task in natural language processing, whose purpose is to identify entity nouns in statements, such as place, person, organization, etc\cite{sharnagat2014named}. The current NER technologies have been mature and widely used in various downstream tasks\cite{goyal2018recent}. Similarly, relation extraction focuses on relationship between entities, which connects two entities semantically, and then represents the semantic information of the target text together with the entities\cite{pawar2017relation, wang2021relation}. However, NER and relation extraction only focus on partial entities and corresponding type information in the text, whose acquired knowledge structure is single and semantic representation ability is poor, thus ignoring other important information, such as a series of actions taken by users in the manuals. 
Event extraction is used to extract structured event information from statements\cite{li2021deep}. An event has three characteristics: trigger words, event types and event arguments. Event extraction is to extract trigger words and arguments from the statements\cite{hogenboom2011overview}. However, event extraction represents the semantic information from a macro perspective, focusing only on the general situation and ignoring the details. In addition, the predicates corresponding to the "attribute descriptions" knowledge does not conform to the definition of event trigger words, making it impossible to use event schema to represent all of knowledge contained in the manuals. 

==> chapters-old/related.tex <==
\section{Related Work}
In this section, we summarize the related work and discuss their connections to our model. We begin with current solutions of knowledge extraction from user instructions, then we briefly introduce existing four-type datasets of user instructions.
% We also discuss the semantic parsing techniques on \kh.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            
\subsection{Knowledge comprehension of user instructions}
Currently, the majority of knowledge comprehension of user instructions focus on procedure comprehension. These works can be grouped into three paradigms: entity-aware state tracking, which targets to identify the state values of the pre-defined entities at each step~\cite{bosselut2017simulating,amini2020procedural,tandon-etal-2020-dataset,goyal2021tracking,zhang2021knowledge}, e.g., predicting the location of tomato at the second step~\cite{zhang2021knowledge}; domain-specific entity 
prediction, which targets to assign the given text span an entity label ~\cite{zhang2012automatically,mysore2019materials,jiang2020recipe,nabizadeh2020myfixit}, e.g., judging whether ``400 degrees F'' is a temperature entity or not~\cite{jiang2020recipe}; 
action-centered graph extraction, which targets to form an action-centered graph with all actions are ordered and all entities are attached to an action~\cite{kiddon_mise_2015,maeta2015framework,vaucher2020automated,kuniyoshi2020annotating,nishimura2020visual}.\par
% , for example, constructing a graph with all nodes are entities or actions, the edge between two action means the next step, and the edge between an entity and an action indicates the condition of the action~\cite{kuniyoshi2020annotating}.
Although these works have gain inference ability over procedure, the overlook of declarative information grounding it makes them lack of a whole comprehension of user instructions.
% and face the issue of ``vicious regresses''~\cite{kieras1984role,karreman2005procedural,ryle2009concept}. We notice a solution for construction regulations pays attention to \kt in user instructions~\cite{zhong2020deep}. However, it only model a certain form of \kt, i.e., an action can be conducted only under a specific condition). 
To break these limitations, we are take the first step the integrated comprehension of user instructions, along with a dense definition of the information on the machine side, a novel corpus, eight baselines, and a standard evaluation method.
\subsection{Datasets of user instructions} 
% short-version
We find four types of existing datasets related to user instructions: the first type annotates domain-specific entities~(e.g., food, action) and verb relations between entities of recipes~\cite{zhang2012automatically,mori2014flow,kiddon_mise_2015,bosselut2017simulating,yamakata2020english,jiang2020recipe}; the second type focuses on technical manuals of device  maintenance~\cite{zhang2012automatically,nabizadeh2020myfixit,goyal2021tracking}, surgical practices~\cite{bombieri-EtAl:2022:LREC}, and constructions regulations~\cite{zhong2020deep}, the annotations involve domain-specific entities~(e.g., action, tool), action relations~(e.g., before, next), action states~(e.g., isOpened), and domain-specific frames; the third type is about scientific experiments~(i.e., material synthesis), \citet{mysore2019materials} labels domain-specific entities and relations of the entities at sentence-level, \citet{vaucher2020automated} annotates the actions in the sentences, \citet{kuniyoshi2020annotating} represents the synthesis process as a flow graph; the last type is the OpenPI dataset~\cite{tandon-etal-2020-dataset}, which annotates the state changes of each sentence from the how-to paragraphs.
% long-version
% We find five types of existing datasets related to user instructions. 
% Recipes: \cite{zhang2012automatically} collects 30 BBC recipes and annotates the recipes into steps, each of which consists of a verb and related information of the verb.  \cite{mori2014flow,yamakata2020english} annotate the name entities~(e.g., food, action) in recipes and the edges between the entities. \cite{kiddon_mise_2015} represents each step of a recipe as an action along with the foods and locations. \cite{bosselut2017simulating} further add state changes of \cite{kiddon_mise_2015}'s dataset. The RISeC dataset~\cite{jiang2020recipe} provides action-level annotations of name entities~(e.g., food, duration) and verb relations to entities. Technical manuals: ~\cite{zhang2012automatically,nabizadeh2020myfixit,zhong2020deep,goyal2021tracking,bombieri-EtAl:2022:LREC}
% navigation:~\cite{macmahon2006walk,shridhar2020alfred} need a map, A instruct B,
% Scientific experiments:~\cite{kuniyoshi2020annotating,vaucher2020automated}

However, all datasets available only annotate the procedure~(e.g., sentences with actions) of user instructions. As far as we know, there lacks a dataset with annotations of both procedural and declarative information of user instructions. As such, we contribute to the first dataset with densely annotations of procedure and the declarative grounding it. Besides, the dataset is  derived from a new type of user instructions, the helping documents in e-commerce. These documents take a significant place in real-world user instructions and are closely related to the service quality. We believe the dataset can advance the progress of automated comprehension systems~(e.g., QA bots) in e-commerce or more.


\subsection{Semantic parsing on user manual\kh}
Before talking about the techniques, it should be noted that the \kh exists not only user instructions but procedures not issued by human. Take the ProPara dataset~\cite{dalvi2018tracking} as an example, it contains scientific processes~(e.g., photosynthesis) whose \kh is issued by entities like water. Along with the ProPara, efforts~\cite{clark2018happened,forbus2018step,ribeiro2019predicting,kazeminejad_automatic_2021,brown2022semantic} have been made to test the potential of verb semantics to structure \kh. It has been experimentally demonstrated that VerbNet~\cite{schuler2005verbnet} or FrameNet~\cite{ruppenhofer2016framenet}) is useful to predict the existence and location of a given entity in ProPara. \par
The above practices inspires us to investigate the relationship between the logical form of knowledge dependency in user instruction and semantic dependency in linguistics. However, we argue both VerbNet and FrameNet are not enough for the knowledge extraction from user instructions due to three issues. First, the arguments in user instructions are more than existences and locations. An action of \kh is along with patients, manner, location, time and notes and the arguments in \kt consist of attributes, relations, etc. Second, the verbs defined in VerbNet and FrameNet are far from complete compared to the world actions. For example, the VerbNet only cover about 40\% actions in ProPara~\cite{clark2018happened}. Third, the knowledge in user instructions is beyond actions. It also involves \kt and how \kt is grounding \kh. To alleviate these issues, \cite{jiang2020recipe,bombieri-EtAl:2022:LREC} chooses to design a new framebank for surgery. But it is domain-specific and needs a big consumption of time and experts. Thus, instead of developing a repository of arguments in \dataname, we design the \model, which model knowledge dependency by semantic parsers and heuristics, to extract complex knowledge from user instructions.
such explorations can neither be extended into the \kh of user instructions because of two reasons. Both VerbNet and FrameNet are far from complete compared to the world actions, for example, the VerbNet only cover about 40\% actions in ProPara~\cite{clark2018happened}.

\cite{forbus2018step}
\cite{ribeiro2019predicting}
\cite{kazeminejad_automatic_2021}
\cite{brown2022semantic}
\cite{bombieri-EtAl:2022:LREC}
\cite{clark2018happened} \cite{kazeminejad_automatic_2021} not user


% ----
It should be noted that the \kh exists in not only user manuals but steps not issued by human. Take the ProPara dataset~\cite{dalvi2018tracking} as an example, it contains scientific processes~(e.g., photosynthesis) whose \kh is issued by entities like water. Along with the ProPara, efforts~\cite{clark2018happened,forbus2018step,ribeiro2019predicting,kazeminejad_automatic_2021,brown2022semantic} have been made to test the potential of verb semantics to structure \kh. It has been experimentally demonstrated that VerbNet~\cite{schuler2005verbnet} or FrameNet~\cite{ruppenhofer2016framenet}) is useful to predict the existence and location of a given entity in ProPara. \par
The above practices inspire us to investigate the relationship between the logical form of the graph in user manuals and semantic dependency in linguistics. However, we argue both VerbNet and FrameNet are not enough for the graph construction from user manuals due to three issues. First, the arguments in user manuals are more than existences and locations. An action of \kh is along with patients, manner, location, time, and modifier and the arguments in \kt consist of attributes, relations, etc. Second, the verbs defined in VerbNet and FrameNet are far from complete compared to the world actions. For example, the VerbNet only covers about 40\% actions in ProPara~\cite{clark2018happened}. Third, the knowledge in user manuals is beyond actions. It also involves \kt and how \kt is binding \kh. To alleviate these issues, \cite{jiang2020recipe,bombieri-EtAl:2022:LREC} chooses to design a new framebank for surgery. But it is domain-specific and needs a big consumption of time and experts. Thus, instead of developing a repository of arguments in \dataname, we design the \model, which models the logical form of the graph by semantic parsers and heuristics, to construct complex graph from user manuals.


==> chapters-old/rep___v1.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{c|c|m{15cm}}
    \hline
      \textbf{Term} &\textbf{Category} & \textbf{Explanation} \\
      \hline
     Action & node & the action of a step performed by the user, presented as a verb, e.g., ``pay''.\\
        \hline
    Entity & node & the unique concepts related to the user manual, e.g., ``scratch card''. Each user manual has a user Entity by default.\\
    \hline
 Action-ARG& argument& the modifier~(\textcolor{orange}{MOD}), time~(\textcolor{orange}{TIME}), location~(\textcolor{orange}{LOC}), manner~(\textcolor{orange}{MANN}), and cause~(\textcolor{orange}{CAUSE}) arguments associated with an Action node. \\
    \hline
    Entity-ARG& argument& the arguments associated with an Entity node --- footnote argument~(\textcolor{NavyBlue}{FN}), offering more details of the entity; attribute argument~(\textcolor{NavyBlue}{ATT}), describing a specific aspect of the entity~(e.g., the hit rate of the scratch card); state argument~(\textcolor{NavyBlue}{STATE}), describing the changeable states of the entity~(e.g., the ``have'' state of the same user). They are derived from the facts binding the steps.\\
    \hline
    ARG-ARG& argument& the arguments associated with an Entity-ARG. The arguments of \textcolor{NavyBlue}{ATT} are the same as Entity-ARG and the arguments of \textcolor{NavyBlue}{STATE} is the same as Action-ARG.\\
        \hline
    
    NEXT & relation & the directed edge between two Action nodes, indicating the end action is the next step of the start one. It determines the order of the actions performed by the user.\\
    \hline
    AGENT&relation& the directed edge from the user Entity node to an Action node, indicating the action is performed by the user.
    % , e.g., the edge from ``user'' to ``pay''.
    \\
    \hline
    PAT& relation& the directed edge from an Action node to an Entity node, indicating the action is performed on the entity.\\
    \hline
    SUB& relation& the directed edge between two Entity nodes, indicating the start entity is a sub-entity of the end one.\\
    \hline
    PATA & relation& the directed edge from a \textcolor{NavyBlue}{STATE} to an Entity node, indicating the entity undergoes the effect caused by the changing of \textcolor{NavyBlue}{STATE}. Note that, the user dominates the whole user manual so that the user Entity cannot be the target of any \textcolor{NavyBlue}{STATE}.\\
    \hline
    \end{tabular}
    }
    \caption{Explanations of nodes, relations, and arguments in the structured representation}
    \label{tab:kg}
\end{table*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/rep.png}
    \caption{Screenshot of the graph obtained from the user manual and the graphs obtained from Q1, Q2, and Q3}
    \label{fig:rep}
\end{figure*}
\section{Structured Representation}
In this section, we will introduce the structured representation to support the unified inference of various types of questions. 
% It is a heterogeneous graph defined as $\mathcal{G}=\{\mathcal{V},\mathcal{R}\}$, where $\mathcal{V}$ is the set of action nodes $\mathcal{V}_A=\{A_i\}_{i=0}^n$ and entity nodes $\mathcal{V}_E=\{E_j\}_{i=0}^m$, $\mathcal{R}$ is the set of action-action, entity-entity, and action-entity relations.

\par
\subsection{Definitions}
The user manual consists of a sequence of steps and a set of facts binding the steps. We propose a structured representation that can describe the steps and facts in a unified graph. The graph is heterogeneous with two kinds of nodes, five kinds of relations, and three kinds of arguments, as defined in Table~\ref{tab:kg}. Based on these definitions, we can represent the user manual in Figure~\ref{fig:style} into a graph, part of which is displayed in Figure~\ref{fig:rep}\footnote{Note that, although the \textcolor{NavyBlue}{STATE} of Entity shares the same arguments with an Action node, it cannot be upgraded into a node because it doesn't refer to an action and cannot be linked to other Action nodes. Similarly, the \textcolor{NavyBlue}{ATT} of an Entity node cannot be upgraded into a node because it can't be linked to other Entity nodes except for the parent one. }. The proposed representation can also be used to map user questions, as shown in the right part of Figure~\ref{fig:rep}.



% Take the user manual in Figure~\ref{fig:style} as an example, it can be represented as a heterogeneous graph, as illustrated in Figure~\ref{fig:rep}.
% which includes  The details 



% We represnet
% Take the user manual in Figure~\ref{fig:style} as an example. It consists of a sequence of six steps and a set of facts binding the steps. \par
% For steps, we assume that each of them consists of an action performed by the user. For instance, S-6 has two user-performed actions, thus it is separated into two steps. Note that, although S-7 has a user-related verb, it cannot be treated as a step because ``have'' doesn't refer to an action. Besides the requisite verb, the action may also have modifier~(\textcolor{orange}{MOD}), time~(\textcolor{orange}{TIME}), location~(\textcolor{orange}{LOC}), manner~(\textcolor{orange}{MANN}), and cause~(\textcolor{orange}{CAUSE}) arguments. As such, a step can be denoted by a user entity, a patient entity, and an action with its arguments. \par
% As for the facts binding the steps, we define them as arguments of the entities. There are three kinds of arguments: footnote argument~(\textcolor{NavyBlue}{FN}), which offers more details of the entity; attribute argument~(\textcolor{NavyBlue}{ATT}), which describes a specific aspect of the entity~(e.g., the hit rate of the scratch card); state argument~(\textcolor{NavyBlue}{STATE}), which describes the changeable states of the entity~(e.g., the ``have'' state of the same user). Specifically, the attribute argument and the state argument share the same structure of the action and entity, respectively. The difference is that they are related to other actions or entities.\par  
% Based on the above assumptions, we define the user manual as a heterogeneous graph with two kinds of nodes with arguments and three groups of relations. The details are as follows.
% \paragraph{Action node}It is an active verb~(e.g., ``sign in'') associated with modifier, time, location, manner, and cause arguments. The arguments can be empty.
% \paragraph{Entity node}It is a concept~(e.g., ``APP'') associated with footnote, attribute, and state arguments. The arguments can be empty. Note that, though the  attribute argument is the same as the entity in format, we don't use it as a node because it isn't linked to other actions and entities. The state argument is not used as a node for the same reason.
% \paragraph{Action-action relation}It is a directed edge between two actions, indicating the end action is the next step~(NEXT) of the start action. 
% \paragraph{Action-entity relation} It is a directed edge between action and entity. If the edge starts from the action, it means the entity is the patient of the action. Otherwise, it means the entity is the agent of the action.
% \paragraph{Entity-Entity relation}It is an edge between two entities indicating they are the same entity or one entity is the sub-entity of the other.
% For example, the 3$^{rd}$ step is denoted as $S_3=\{\text{user --> pay --> NULL; MANN: scan the QR code}\}$
% Formally, a step is denoted as a triple $\mathcal{S}=\{user, \}$
% % $A=\(\text{VERB; MOD | TIME | LOC | MANN | CAUSE}\)$



% For simplicity, 
% The representation is a heterogeneous graph with two kinds of nodes~(action node and entity node) and three groups of relations. 
% \paragraph{Nodes}

\subsection{Unified Inference}
The proposed representation is able to support the unified inference of various types of user questions.

==> tables-old/QA_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{CJK}{UTF8}{gbsn}
\begin{table*}[]
\scalebox{0.6}{
\renewcommand\arraystretch{1.2}
\begin{tabular}{c|l}
\hline
\multirow{23}{*}{Document}             & 钉钉用户个人信息修改指南                                                                                                                                                                                                                \\
                                       & DingTalk User Personal Information Amendment Guide      \\&                                                                                                                                                                    \\
                                       & 您好，若需要修改个人信息，按照如下方法操作：                                                                                                                                                                                                      \\
                                       & Hello, if you need to modify your personal information, please follow the steps below:                                                                                                                                      \\
                                       & {\color[HTML]{00C957}点开自己的个人资料页面，拉到底部}可以按部门要求设置昵称，电脑端暂不支持设置头像、钉钉号等信息。                                                                                                                                                                             \\
                                       & {\color[HTML]{00C957}Click on your personal profile page, scroll down to the bottom} and set nicknames according to department requirements. \\& The computer side does not support setting profile pictures, DingTalk numbers and other information. \\
                                       & 【温馨提示】                                                                                                                                                                                                                      \\
                                       & 【Kind tips】                                                                                                                                                                                                                 \\
                                       & 1、若选择恢复默认头像，则头像默认显示昵称最后的几个字，头像背景颜色随机，不支持自定义选择颜色；                                                                                                                                                                            \\
                                       & 1. If you choose to restore the default avatar, the avatar will display the last few words of the nickname by default, \\&and the background color of the avatar is random, and custom selection of color is not supported;    \\
                                       & 2、昵称是自己设置的，管理员等其他人无权修改，管理员可以在企业通讯录里设置员工在企业内的名称；                                                                                                                                                                             \\
                                       & 2. The nickname is set by oneself, the administrator and others have no right to modify it, the administrator can set the \\& name of the employee in the enterprise in the enterprise address book;                            \\
                                       & 3、个人昵称的字数限制在20字以内，更换头像没有限制；                                                                                                                                                                                                 \\
                                       & 3. The number of characters in the personal nickname is limited to 20 characters, and there is no limit to changing the avatar;                                                                                             \\
                                       & 4、管理员在“管理后台-通讯录”中修改员工名字字符不超过80个字符；                                                                                                                                                                                          \\
                                       & 4. The administrator can modify the employee's name to no more than 80 characters in the "Management Background-Contact Book";                                                                                              \\
                                       & 5、若您是在班级群内的姓名显示不对，需要联系对应班级的班主任进行修改哦。                                                                                                                                                                                        \\
                                       & 5. If your name in the class group is displayed incorrectly, you need to contact the head teacher of the corresponding class to modify it.                                                                                  \\ \hline
\multirow{2}{*}{Question}              & {\color[HTML]{FF9912}在哪里设置昵称}                                                                                                                                                                                                                     \\
                                       & {\color[HTML]{FF9912}where to set nickname}                                                                                                                                                                                                       \\ \hline
\multirow{2}{*}{Answer by Graph Match} & {\color[HTML]{00C957}点开自己的个人资料页面，拉到底部}                                                                                                                                                                                                            \\
                                       & {\color[HTML]{00C957}Click on your profile page, scroll to the bottom} 
                                       \\ \hline
\multirow{2}{*}{Answer by Chinese Word Vector} & 按部门要求设置昵称                                                                                                                                                                                                            \\
                                       & set nicknames according to department requirements 
                                       \\ \hline
\multirow{2}{*}{Answer by Keywords Window} & 昵称是自己设置的 \quad|\quad 个人昵称的字数限制在20字以内                                                                                                                                                                                                          \\
                                       & The nickname is set by oneself \quad|\quad The number of characters in the personal nickname is limited to 20 characters 
                                       \\ \hline
\end{tabular}
}
\caption{Example demonstration of Question Answering. Here is the text of the question, the document sentences used to find the answer, and the answers given by several different models.}
\label{tab:QA_example}
\end{table*}
\end{CJK}

==> tables-old/QA_factoid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{ulem}

\begin{table*}
\centering
\scalebox{0.75}{
\begin{tabular}{r|c|ccc|ccc}
\multicolumn{1}{c|}{Baseline}                  & question match rate & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall}    & \multicolumn{1}{c}{F1} &
\multicolumn{1}{|c}{Precision@1} & \multicolumn{1}{c}{Recall@1}    & \multicolumn{1}{c}{F1@1}
\\ \hline
\multicolumn{1}{l|}{\textbf{SurfacePatternMatching}}    &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-User Instruction Pattern} & 94.3\%              & \underline{0.7889}                  & 0.2785                        & 0.4116  &
\underline{0.7889}                  & 0.2785                        & 0.4116
\\ \hline
\multicolumn{1}{l|}{\textbf{LexicalMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-BLEU}                             & -                   & 0.3458                        & 0.4699                        & 0.3984 &
0.3600                        & 0.3166                        & 0.3369 \\
\multicolumn{1}{l|}{\qquad-Edit Distance}                           & -                   & 0.4792                        & 0.5871                        & 0.5277
& 0.5379                        & 0.4800                        & 0.5073
\\ \hline
\multicolumn{1}{l|}{\textbf{SemanticMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Bert Base}                             & -       
& 0.3844                        & 0.6171                        & 0.4737
& 0.4157                        & 0.3745                        & 0.3940                        \\
\multicolumn{1}{l|}{\qquad-Char CNN}                           & -       
& 0.3350                        & 0.5442                        & 0.4147
& 0.3226                        & 0.2938                        & 0.3075                        \\
\multicolumn{1}{l|}{\qquad-Chinese Word Vectors}                           & -     
& 0.4654    & \underline{0.7323} & 
\underline{0.5691}
& 0.5767                        & \underline{0.5087}   & \underline{0.5406}                        \\
\multicolumn{1}{l|}{\qquad-Bert Score}                           & -   
& 0.4610                        & 0.7269                        & 0.5642
& 0.5611                        & 0.4986                        & 0.5281                        \\
\hline
\multicolumn{1}{l|}{\textbf{KeywordsMatching}}          &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Synonyms Plus}            & -                   
& 0.4263                        & 0.6642                        & 0.5193 
& 0.4661                        & 0.4111                        & 0.4369 \\
\multicolumn{1}{l|}{\qquad-Keywords Window}          & -                   
& 0.4635  & 0.7271 & 0.5662
& 0.5587  & 0.4917  & 0.5231
\\ \hline
\multicolumn{1}{l|}{\textbf{PLM}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Macbert Large}                                & -                   & 0.1111                        & 0.1121                        & 0.1116
& 0.1111                        & 0.1121                        & 0.1116 \\
\multicolumn{1}{l|}{\qquad-Pert Large}                                   & -                   & 0.2628                        & 0.2423                        & 0.2522
& 0.2628                        & 0.2423                        & 0.2522 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm}                                  & -                   & 0.1226                        & 0.1265                        & 0.1245
& 0.1226                        & 0.1265                        & 0.1245 \\ \hline
\multicolumn{1}{l|}{\textbf{SelfSupervised}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Pert Large w/ self supervision}   & -
& 0.3650                        & 0.2771                        & 0.3150
& 0.3150                        & 0.2771                        & 0.3150 \\
\multicolumn{1}{l|}{\qquad-Macbert Large w/ self supervision}   & -
& 0.3900                        & 0.3075                        & 0.3439
& 0.3900                        & 0.3075                        & 0.3439 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm w/ self supervision}   & -
& 0.4396                        & 0.3599                        & 0.3958
& 0.4396                        & 0.3599                        & 0.3958 \\
\hline
\multicolumn{1}{c|}{ours}                                          & 93.4\%                   & {\color[HTML]{FE0000} 0.8618} & 
{\color[HTML]{FE0000} 0.7804}                  & {\color[HTML]{FE0000} 0.8191} &
{\color[HTML]{FE0000} 0.8778} & {\color[HTML]{FE0000} 0.6690}                  & {\color[HTML]{FE0000} 0.7593}
\end{tabular}
}
\caption{Results of the baseline approaches on Experiment \Rmnum{2} for Factoid-style questions. The question matching rate shows the recognition rate of some baselines for question types. We first evaluated the precision, recall and F1 scores of each baseline under its optimal settings. Then, for the sake of fairness, we evaluated the scores of each baseline when the hit ratio of the answer is set to 1. The best results are marked in red, and the second best results are marked by underline.}
\label{tab:exp2_factoid}
\end{table*}

==> tables-old/QA_fine-tune_PLM.tex <==
\begin{table*}
\centering
\scalebox{0.85}{
\begin{tabular}{l|c|c|c|c|c|c}
\multicolumn{1}{c|}{Models} & Precision & Recall & F1     & Precision@1 & Recall@1 & F1@1   \\ \hline
\qquad-Pert Large w/ fine-tune    & 0.5724    & 0.2581 & 0.3558 & 0.6364      & 0.2327   & 0.3408 \\ \hline
\qquad-Macbert Large w/ fine-tune & 0.4932    & 0.4546 & 0.4731 & 0.6191      & 0.3746   & 0.4668 \\ \hline
\qquad-Roberta wwm w/ fine-tune   & 0.5591    & 0.2644 & 0.3590 & 0.6216      & 0.2364   & 0.3425 \\ \hline
\end{tabular}
}
\caption{Experimental results of the fine-tune models. We evaluated the accuracy, recall and F1 scores of all models on the test set. Because the test set used by the fine-tune models is not completely consistent with the test set used by other models mentioned above (only half of the annotated QA data as the test set), the experimental results of the fine-tune models are listed separately. Similarly, in order to make a fair comparison, we also conducted experiments under the condition of limiting the hit ratio of the answer is set to 1.}
\label{tab:exp2_fine_tune}
\end{table*}


==> tables-old/QA_inconsistency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{ulem}

\begin{table*}
\centering
\scalebox{0.75}{
\begin{tabular}{r|c|ccc|ccc}
\multicolumn{1}{c|}{Baseline}                  & question match rate & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall}    & \multicolumn{1}{c}{F1} &
\multicolumn{1}{|c}{Precision@1} & \multicolumn{1}{c}{Recall@1}    & \multicolumn{1}{c}{F1@1}
\\ \hline
\multicolumn{1}{l|}{\textbf{SurfacePatternMatching}}    &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-User Instruction Pattern} & 71.9\%              & {\color[HTML]{FE0000} 0.8534}                  & 0.1842                        & 0.3029  &
\underline{0.8534}                  & 0.1842                        & 0.3029
\\ \hline
\multicolumn{1}{l|}{\textbf{LexicalMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-BLEU}                             & -                   & 0.3204                        & 0.4331                        & 0.3683 &
0.3584                        & 0.3171                        & 0.3364 \\
\multicolumn{1}{l|}{\qquad-Edit Distance}                           & -                   & 0.4851                        & 0.5670                        & 0.5228
& 0.5513                        & 0.4928                        & 0.5204
\\ \hline
\multicolumn{1}{l|}{\textbf{SemanticMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Bert Base}                             & -       
& 0.3758                        & 0.6074                        & 0.4643
& 0.4065                        & 0.3698                        & 0.3873                        \\
\multicolumn{1}{l|}{\qquad-Char CNN}                           & -       
& 0.3200                        & 0.5244                        & 0.3975
& 0.3009                        & 0.2773                        & 0.2886                        \\
\multicolumn{1}{l|}{\qquad-Chinese Word Vectors}                           & -     
& 0.4710                        & {\color[HTML]{FE0000} 0.7430} & \underline{0.5766}
& 0.5963                        & \underline{0.5287}   & \underline{0.5605}                        \\
\multicolumn{1}{l|}{\qquad-Bert Score}                           & -   
& 0.4675                        & \underline{0.7393}                        & 0.5728
& 0.5739                        & 0.5135                        & 0.5420                        \\
\hline
\multicolumn{1}{l|}{\textbf{KeywordsMatching}}          &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Synonyms Plus}            & -                   
& 0.4534                        & 0.6828                        & 0.5449 
& 0.5083                        & 0.4440                        & 0.4740 \\
\multicolumn{1}{l|}{\qquad-Keywords Window}          & -                   
& 0.4712  & 0.7377 & 0.5751
& 0.5765  & 0.5102  & 0.5413
\\ \hline
\multicolumn{1}{l|}{\textbf{PLM}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Macbert Large}                                & -                   & 0.1420                        & 0.1417                        & 0.1418
& 0.1420                        & 0.1417                        & 0.1418 \\
\multicolumn{1}{l|}{\qquad-Pert Large}                                   & -                   & 0.2764                        & 0.2618                        & 0.2689
& 0.2764                        & 0.2618                        & 0.2689 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm}                                  & -                   & 0.1561                        & 0.1554                        & 0.1557
& 0.1561                        & 0.1554                        & 0.1557 \\ \hline
\multicolumn{1}{l|}{\textbf{SelfSupervised}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Pert Large w/ self supervision}   & -
& 0.3760                        & 0.2936                        & 0.3298
& 0.3760                        & 0.2936                        & 0.3298 \\
\multicolumn{1}{l|}{\qquad-Macbert Large w/ self supervision}   & -
& 0.4039                        & 0.3290                        & 0.3626
& 0.4039                        & 0.3290                        & 0.3626 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm w/ self supervision}   & -
& 0.4350                        & 0.3632                        & 0.3958
& 0.4350                        & 0.3632                        & 0.3958 \\
\hline
\multicolumn{1}{c|}{ours}                                          & 85.2\%        & \underline{0.8492}  & 0.6750          & {\color[HTML]{FE0000} 0.7522} &
{\color[HTML]{FE0000} 0.8809} & {\color[HTML]{FE0000} 0.5912}                  & {\color[HTML]{FE0000} 0.7075}
\end{tabular}
}
\caption{Results of the baseline approaches on Experiment \Rmnum{2} for Inconsistent questions. The question matching rate shows the recognition rate of some baselines for question types. We first evaluated the precision, recall and F1 scores of each baseline under its optimal settings. Then, for the sake of fairness, we evaluated the scores of each baseline when the hit ratio of the answer is set to 1. The best results are marked in red, and the second best results are marked by underline.}
\label{tab:exp2_inconsistent}
\end{table*}

==> tables-old/QA_procedure.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{ulem}

\begin{table*}
\centering
\scalebox{0.75}{
\begin{tabular}{r|c|ccc|ccc}
\multicolumn{1}{c|}{Baseline}                  & question match rate & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall}    & \multicolumn{1}{c}{F1} &
\multicolumn{1}{|c}{Precision@1} & \multicolumn{1}{c}{Recall@1}    & \multicolumn{1}{c}{F1@1}
\\ \hline
\multicolumn{1}{l|}{\textbf{SurfacePatternMatching}}    &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-User Instruction Pattern} & 79.6\%              & \underline{0.7550}                  & 0.2643                        & 0.3915  &
\underline{0.7550}                  & 0.2643                        & 0.3915
\\ \hline
\multicolumn{1}{l|}{\textbf{LexicalMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-BLEU}                             & -                   & 0.3166                        & 0.4303                        & 0.3648 &
0.3575                        & 0.3216                        & 0.3386 \\
\multicolumn{1}{l|}{\qquad-Edit Distance}                           & -                   & 0.4609                        & 0.5732                        & 0.5110
& 0.5107                        & 0.4644                        & 0.4864
\\ \hline
\multicolumn{1}{l|}{\textbf{SemanticMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Bert Base}                             & -       
& 0.3727                        & 0.6152                        & 0.4642
& 0.3948                        & 0.3644                        & 0.3790                        \\
\multicolumn{1}{l|}{\qquad-Char CNN}                           & -       
& 0.3276                        & 0.5458                        & 0.4095
& 0.3052                        & 0.2845                        & 0.2945                        \\
\multicolumn{1}{l|}{\qquad-Chinese Word Vectors}                           & -     
& 0.4642   & \underline{0.7546} & 0.5748
& 0.5809                        & \underline{0.5189}   & \underline{0.5481}                        \\
\multicolumn{1}{l|}{\qquad-Bert Score}                           & -   
& 0.4594                        & 0.7475                        & 0.5691
& 0.5588                        & 0.5086                        & 0.5325                        \\
\hline
\multicolumn{1}{l|}{\textbf{KeywordsMatching}}          &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Synonyms Plus}            & -                   
& 0.4276                        & 0.6655                        & 0.5206 
& 0.4847                        & 0.4300                        & 0.4557 \\
\multicolumn{1}{l|}{\qquad-Keywords Window}          & -                   
& 0.4666  & {\color[HTML]{FE0000}0.7578} & \underline{0.5776}
& 0.5793  & 0.5182  & 0.5470
\\ \hline
\multicolumn{1}{l|}{\textbf{PLM}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Macbert Large}                                & -                   & 0.1027                        & 0.1111                        & 0.1067
& 0.1027                        & 0.1111                        & 0.1067 \\
\multicolumn{1}{l|}{\qquad-Pert Large}                                   & -                   & 0.2390                        & 0.2356                        & 0.2373
& 0.2390                        & 0.2356                        & 0.2373 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm}                                  & -                   & 0.1091                        & 0.1223                        & 0.1153
& 0.1091                        & 0.1223                        & 0.1153 \\ \hline
\multicolumn{1}{l|}{\textbf{SelfSupervised}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Pert Large w/ self supervision}   & -
& 0.3592                        & 0.2812                        & 0.3155
& 0.3150                        & 0.2771                        & 0.3150 \\
\multicolumn{1}{l|}{\qquad-Macbert Large w/ self supervision}   & -
& 0.3895                        & 0.3197                        & 0.3512
& 0.3895                        & 0.3197                        & 0.3512 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm w/ self supervision}   & -
& 0.3999                        & 0.3304                        & 0.3618
& 0.3999                        & 0.3304                        & 0.3618 \\
\hline
\multicolumn{1}{c|}{ours}                                          & 89.9\%                   & {\color[HTML]{FE0000} 0.8637} & 0.7500                  & {\color[HTML]{FE0000} 0.8028} &
{\color[HTML]{FE0000} 0.8979} & {\color[HTML]{FE0000} 0.6372}                  & {\color[HTML]{FE0000} 0.7454}
\end{tabular}
}
\caption{Results of the baseline approaches on Experiment \Rmnum{2} for Procedural-style questions. The question matching rate shows the recognition rate of some baselines for question types. We first evaluated the precision, recall and F1 scores of each baseline under its optimal settings. Then, for the sake of fairness, we evaluated the scores of each baseline when the hit ratio of the answer is set to 1. The best results are marked in red, and the second best results are marked by underline.}
\label{tab:exp2_procedure}
\end{table*}

==> tables-old/QA_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{ulem}

\begin{table*}
\centering
\scalebox{0.77}{
\begin{tabular}{r|c|ccc|ccc}
\multicolumn{1}{c|}{Method}               &   &  \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall}    & \multicolumn{1}{c}{F1} &
\multicolumn{1}{|c}{Precision@1} & \multicolumn{1}{c}{Recall@1}    & \multicolumn{1}{c}{F1@1}
\\ \hline
\multicolumn{1}{l|}{\textbf{SurfacePatternMatching}}  &  &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-User Instruction Pattern} &\%              & \underline{0.7679}                  & 0.1833                        & 0.2959  &
\underline{0.7679}                  & 0.1833                        & 0.2959
\\ \hline
\multicolumn{1}{l|}{\textbf{LexicalMatching}}                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-BLEU}                             & -                   & 0.3084                        & 0.4323                        & 0.3600 &
0.3361                        & 0.3077                        & 0.3213 \\
\multicolumn{1}{l|}{\qquad-Edit Distance}                           & -                   & 0.4473                        & 0.5604                        & 0.4975
& 0.4965                        & 0.4610                        & 0.4781
\\ \hline
\multicolumn{1}{l|}{\textbf{SemanticMatching}}           &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Bert Base}                             & -       
& 0.3584                        & 0.6006                        & 0.4489
& 0.3774                        & 0.3557                        & 0.3662                        \\
\multicolumn{1}{l|}{\qquad-Char CNN}                           & -       
& 0.3125                        & 0.5284                        & 0.3928
& 0.2896                        & 0.2757                        & 0.2825                        \\
\multicolumn{1}{l|}{\qquad-Chinese Word Vectors}                           & -     
& 0.4493                        & {\color[HTML]{FE0000} 0.7399} & \underline{0.5591}
& 0.5502                        & \underline{0.5032}   & \underline{0.5257}                        \\
\multicolumn{1}{l|}{\qquad-Bert Score}                           & -   
& 0.4435                        & 0.7317                        & 0.5523
& 0.5268                        & 0.4881                        & 0.5067                        \\
\hline
\multicolumn{1}{l|}{\textbf{KeywordsMatching}}          &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Synonyms Plus}            & -                   
& 0.4181                        & 0.6652                        & 0.5134 
& 0.4591                        & 0.4158                        & 0.4364 \\
\multicolumn{1}{l|}{\qquad-Keywords Window}          & -                   
& 0.4486  & \underline{0.7358} & 0.5574
& 0.5400  & 0.4933  & 0.5156
\\ \hline
\multicolumn{1}{l|}{\textbf{PLM}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Macbert Large}                                & -                   & 0.1124                        & 0.1185                        & 0.1154
& 0.1124                        & 0.1185                        & 0.1154 \\
\multicolumn{1}{l|}{\qquad-Pert Large}                                   & -                   & 0.2412                        & 0.2362                        & 0.2387
& 0.2412                        & 0.2362                        & 0.2387 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm}                                  & -                   & 0.1253                        & 0.1355                        & 0.1302
& 0.1253                        & 0.1355                        & 0.1302 \\ \hline
\multicolumn{1}{l|}{\textbf{SelfSupervised}}                       &                     &                               &                               &                               \\
\multicolumn{1}{l|}{\qquad-Pert Large w/ self supervision}   & -
& 0.4111                        & 0.3424                        & 0.3736
& 0.4111                        & 0.3424                        & 0.3736 \\
\multicolumn{1}{l|}{\qquad-Macbert Large w/ self supervision}   & -
& 0.4354                        & 0.3671                        & 0.3984
& 0.4354                        & 0.3671                        & 0.3984 \\
\multicolumn{1}{l|}{\qquad-Roberta wwm w/ self supervision}   & -
& 0.3969                        & 0.3347                        & 0.3632
& 0.3969                        & 0.3347                        & 0.3632 \\
\hline
\multicolumn{1}{c|}{ours}                                          & 94.4\%                   & {\color[HTML]{FE0000} 0.8875} & 0.6658                  & {\color[HTML]{FE0000} 0.7608} &
{\color[HTML]{FE0000} 0.8708} & {\color[HTML]{FE0000} 0.6115}                  & {\color[HTML]{FE0000} 0.7185}
\end{tabular}
}
\caption{Results of the baseline approaches on Experiment \Rmnum{2}. The question matching rate shows the recognition rate of some baselines for question types. We first evaluated the precision, recall and F1 scores of each baseline under its optimal settings. Then, for the sake of fairness, we evaluated the scores of each baseline when the hit ratio of the answer is set to 1. The best results are marked in red, and the second best results are marked by underline.}
\label{tab:exp2}
\end{table*}

==> tables-old/arguments_extraction_performance.tex <==
\begin{table*}
\centering

% \scalebox{0.75}{
\begin{tabular}{|c|c|ccc|cccc|}

%\textbf{\centering{Experiment results}} \\
\multicolumn{9}{c}{Arguments Extraction}\\
\hline
\multicolumn{2}{|c|}{ \multirow{2}*{Model}} & \multicolumn{3}{c|}{exact match} & \multicolumn{4}{c|}{BLEU}\\
% 用\multicolumn{3}表示横向合并三列
\cline{3-9}
\multicolumn{2}{|c|}{} & \textbf{precision} & \textbf{recall} & \textbf{f1-score} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4}\\
\hline
Pattern Match based & \textbf{PMRD} & \textsc{0.1148} & \textsc{0.0807} & \textsc{0.0948} & \textsc{0.1906} & \textsc{0.1682} & \textsc{0.0580} & \textsc{0.0042}\\
\cline{1-9}
\multirow{4}*{Parser Transformation based} & \textbf{DepT} & \verb|0.7885| & \verb|0.4136| & \verb|0.5426| & \verb|0.4428| & \verb|0.4476| & \verb|0.4727| & \verb|0.4747|\\
\cline{2-9}
 & \textbf{SrlT} & \verb|0.6236| & \verb|0.4358| & \verb|0.5131| & \verb|0.4762| & \verb|0.4810| & \verb|0.5200| & \verb|0.5165|\\
\cline{2-9}
 & \textbf{SdgpT} & \verb|0.5918| & \verb|0.3940| & \verb|0.4731| & \verb|0.4569| & \verb|0.4468| & \verb|0.4378| & \verb|0.4343|\\
\cline{2-9}
 & \textbf{DsdgpT} & \verb|0.6788| & \verb|0.5534| & \verb|0.6097| & \verb|0.6088| & \verb|0.6023| & \verb|0.6077| & \verb|0.6083|\\
\hline

\end{tabular}
% }
\caption{Arguments extraction performance of the proposed baselines.
}
\end{table*}

==> tables-old/core_predicates_identification.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|}
\multicolumn{3}{c}{Core Predicates Identification}\\
\hline
\multicolumn{2}{|c|}{Model} & precision\\
\hline
Pattern Match based & \verb|PMRD| & \verb|0.9466|\\
\hline
\multirow{4}*{Parser Transformation based} & \verb|DepT| & \verb|0.9621|\\
\cline{2-3}
& \verb|SrlT| & \verb|0.9005|\\
\cline{2-3}
& \verb|SdgpT| & \verb|0.8064|\\
\cline{2-3}
& \verb|DsdgpT| & \verb|0.9621|\\
\hline

\end{tabular}
\caption{Core predicates identification precision of the proposed baselines.
}
\end{table*}

==> tables-old/exp1.tex <==
% Table generated by Excel2LaTeX from sheet 'experiment I'
\begin{table*}[t]
  \centering
  \caption{Results of the eight baseline approaches on Experiment \Rmnum{1}. Except for HD and LD, the higher value indicates the better performance. The third column shows the upper bounds of all metrics made by human. The best results of baseline approaches are marked in bold and the second best results are marked by underline.}
  \scalebox{0.88}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \toprule
    \multicolumn{2}{|c|}{} & Human & \multicolumn{1}{c|}{Biafiine-\khs} & \multicolumn{1}{c|}{MFVI-\khs} & HanLP-\khs & \multicolumn{1}{c|}{LTP-\khs} & \multicolumn{1}{c|}{Biafiine-\kts} & \multicolumn{1}{c|}{MFVI-\kts} & \multicolumn{1}{c|}{HanLP-\kts} & \multicolumn{1}{c|}{LTP-\kts} \\
    \midrule
    \multirow{3}[6]{*}{\texttt{Q1}} & P$^\dag$ & 1.00  & 0.20  & 0.19  & \multicolumn{1}{c|}{0.19} & \multicolumn{1}{c|}{\underline{0.27}} & 0.25  & 0.21  & \multicolumn{1}{c|}{0.22} & \multicolumn{1}{c|}{\textbf{0.30}} \\
\cmidrule{2-11}          & R$^\dag$ & 0.98  & 0.37  & 0.44  & \underline{0.79} & 0.62  & 0.39  & 0.45  & \textbf{0.81} & 0.63 \\
\cmidrule{2-11}          & F1$^\dag$ & 0.99  & 0.26  & 0.27  & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\underline{0.37}} & 0.30  & 0.28  & \multicolumn{1}{c|}{0.34} & \multicolumn{1}{c|}{\textbf{0.41}} \\
    \midrule
    \multirow{3}[6]{*}{\texttt{Q2}} & P$^\dag$ & 0.95  & 0.13  & 0.20  & \multicolumn{1}{c|}{0.18} & \multicolumn{1}{c|}{\underline{0.22}} & 0.15  & 0.21  & \underline{0.23} & \multicolumn{1}{c|}{\textbf{0.24}} \\
\cmidrule{2-11}          & R$^\dag$ & 0.89  & 0.14  & 0.29  & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{\underline{0.35}} & 0.17  & 0.30  & \multicolumn{1}{c|}{0.32} & \multicolumn{1}{c|}{\textbf{0.38}} \\
\cmidrule{2-11}          & F1$^\dag$ & 0.92  & 0.14  & 0.24  & \multicolumn{1}{c|}{0.22} & \multicolumn{1}{c|}{\underline{0.27}} & 0.16  & 0.25  & \underline{0.27} & \multicolumn{1}{c|}{\textbf{0.29}} \\
    \midrule
     \multirow{2}[4]{*}{\texttt{Q3}} & HD & 0.02  & 2.32  & 2.05  & \underline{0.79} & 1.47  & 2.13  & 1.95  & \textbf{0.69} & 1.36 \\
\cmidrule{2-11}          & LD & 0.03  & \multicolumn{1}{c|}{\underline{0.66}} & 0.76  & \multicolumn{1}{c|}{1.29} & 0.87  & \multicolumn{1}{c|}{\textbf{0.63}} & 0.71  & \multicolumn{1}{c|}{1.16} & 0.79 \\
    \midrule
    \multirow{3}[6]{*}{\texttt{Q4}} & P$^\dag$ & 0.90  & 0.21  & \multicolumn{1}{c|}{\underline{0.42}} & \multicolumn{1}{c|}{0.28} & 0.36  & 0.24  & \multicolumn{1}{c|}{\textbf{0.46}} & \multicolumn{1}{c|}{0.28} & 0.40 \\
\cmidrule{2-11}          & R$^\dag$ & 0.98  & 0.08  & 0.13  & \multicolumn{1}{c|}{0.14} & \multicolumn{1}{c|}{\underline{0.19}} & 0.09  & 0.14  & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{\textbf{0.20}} \\
\cmidrule{2-11}          & F1$^\dag$ & 0.94  & 0.11  & 0.19  & \multicolumn{1}{c|}{0.19} & \multicolumn{1}{c|}{\underline{0.25}} & 0.14  & 0.21  & \multicolumn{1}{c|}{0.20} & \multicolumn{1}{c|}{\textbf{0.27}} \\
    \midrule
    
    \multirow{3}[6]{*}{\texttt{Q5}} & P$^\dag$ & 0.88  & 0.07  & \multicolumn{1}{c|}{\underline{0.21}} & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{\underline{0.21}} & 0.08  & \multicolumn{1}{c|}{\underline{0.21}} & \multicolumn{1}{c|}{0.17} & \multicolumn{1}{c|}{\textbf{0.22}} \\
\cmidrule{2-11}          & R$^\dag$ & 0.80  & 0.01  & 0.03  & \multicolumn{1}{c|}{0.03} & \multicolumn{1}{c|}{\underline{0.06}} & 0.03  & 0.04  & \multicolumn{1}{c|}{0.05} & \multicolumn{1}{c|}{\textbf{0.07}} \\
\cmidrule{2-11}          & F1$^\dag$ & 0.84  & 0.02  & 0.05  & \multicolumn{1}{c|}{0.06} & \multicolumn{1}{c|}{\underline{0.09}} & 0.04  & 0.07  & \multicolumn{1}{c|}{0.08} & \multicolumn{1}{c|}{\textbf{0.10}} \\
    \midrule
   
    \multirow{3}[6]{*}{\texttt{Q6}} & P     & 0.95  & 0.15  & \multicolumn{1}{c|}{\underline{0.16}} & \multicolumn{1}{c|}{0.13} & 0.09  & \multicolumn{1}{c|}{\underline{0.16}} & \multicolumn{1}{c|}{\textbf{0.17}} & \multicolumn{1}{c|}{0.14} & 0.10 \\
\cmidrule{2-11}          & R     & 0.88  & 0.06  & 0.10  & \underline{0.17} & 0.12  & 0.07  & 0.11  & \textbf{0.18} & 0.13 \\
\cmidrule{2-11}          & F1    & 0.91  & 0.08  & 0.12  & \underline{0.15} & 0.10  & 0.09  & 0.13  & \textbf{0.16} & 0.11 \\
    \midrule
    \multirow{3}[6]{*}{\texttt{Q7}} & P     & 0.79  & 0.12  & \multicolumn{1}{c|}{\underline{0.13}} & \multicolumn{1}{c|}{0.11} & 0.08  & 0.12  & \multicolumn{1}{c|}{\textbf{0.14}} & \multicolumn{1}{c|}{0.12} & 0.08 \\
\cmidrule{2-11}          & R     & 0.70  & 0.05  & 0.07  & \underline{0.13} & 0.10  & 0.06  & 0.07  & \textbf{0.15} & 0.10 \\
\cmidrule{2-11}          & F1    & 0.74  & 0.07  & 0.09  & \underline{0.12} & 0.09  & 0.08  & 0.09  & \textbf{0.13} & 0.09 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:exp1}%
  \vspace{-0.6cm}
\end{table*}%


==> tables-old/human_evaluation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \scalebox{0.77}{
        \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \toprule
    \multicolumn{1}{|r|}{} & \multicolumn{10}{c|}{Wins \%} \\
    \cline{2-11}
    \multicolumn{1}{|r|}{} & \multicolumn{1}{l|}{\begin{turn}{90}PERT$_\text{base}$\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}PERT$_\text{large}$\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}Binafiine-KH\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}MFVI/LBP-KH\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}LTP-KH\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}HanLP-KH\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}Binafiine-KT\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}MFVI/LBP-KT\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}LTP-KT\end{turn}} & \multicolumn{1}{l|}{\begin{turn}{90}HanLP-KT\end{turn}} \\
    \midrule
    \multicolumn{1}{|l|}{PERT$_\text{base}$} & -     & \cellcolor[rgb]{ .686,  .839,  .545}51 & \cellcolor[rgb]{ 1,  .937,  .612}10 &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{|l|}{PERT$_\text{large}$} & \cellcolor[rgb]{ .714,  .851,  .553}47 & -     & \cellcolor[rgb]{ 1,  .937,  .612}10 &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{|l|}{Binafiine-KH} & \cellcolor[rgb]{ .388,  .745,  .482}89 & \cellcolor[rgb]{ .388,  .745,  .482}89 & -     &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{|l|}{MFVI/LBP-KH} &       &       &       & -     &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{|l|}{LTP-KH} &       &       &       &       & -     &       &       &       &       &  \\
    \midrule
    HanLP- KH &       &       &       &       &       & -     &       &       &       &  \\
    \midrule
    \multicolumn{1}{|l|}{Binafiine-KT} &       &       &       &       &       &       & -     &       &       &  \\
    \midrule
    \multicolumn{1}{|l|}{MFVI/LBP-KT} &       &       &       &       &       &       &       & -     &       &  \\
    \midrule
    \multicolumn{1}{|l|}{LTP-KT} &       &       &       &       &       &       &       &       & -     &  \\
    \midrule
    HanLP-KT &       &       &       &       &       &       &       &       &       & - \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table}%


==> tables-old/knowledge_type_judgement.tex <==
\begin{table*}
\centering

\begin{tabular}{|c|c|c|}

\multicolumn{3}{c}{Knowledge Type Judgement}\\
\hline
\multicolumn{2}{|c|}{Model} & precision\\
\hline
Pattern Match based & \verb|PMRD| & \verb|0.9466|\\
\hline
\multirow{4}*{Parser Transformation based} & \verb|DepT| & \verb|0.9621|\\
\cline{2-3}
& \verb|SrlT| & \verb|0.9005|\\
\cline{2-3}
& \verb|SdgpT| & \verb|0.8064|\\
\cline{2-3}
& \verb|DsdgpT| & \verb|0.9621|\\
\hline

\end{tabular}
    \caption{Knowledge type judgement performance of the proposed baselines}
    \label{tab:Knowledge_type_judgement}
\end{table*}

==> tables-old/parsers_trans_rules.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|l|l|l|l|}
\hline
model                                        & knowledge type                                                                     & tags of parser                                             & target arguments                                                                                        & meaning of the argument                                                                 \\ \hline
\multirow{6}{*}{DepT}                        & \multirow{4}{*}{user actions}                                                      & \begin{tabular}[c]{@{}l@{}}SBV\\ FOB\end{tabular}          & argument1                                                                                               & \begin{tabular}[c]{@{}l@{}}the subject who sends\\ out the specific action\end{tabular} \\ \cline{3-5} 
                                             &                                                                                    & VOB                                                        & argument2                                                                                               & \begin{tabular}[c]{@{}l@{}}the object undergoing\\ the specific action\end{tabular}     \\ \cline{3-5} 
                                             &                                                                                    & IOB                                                        & \begin{tabular}[c]{@{}l@{}}become argument2 while\\ fuse primary one with\\ core predicate\end{tabular} & \begin{tabular}[c]{@{}l@{}}the object undergoing\\ the specific action\end{tabular}     \\ \cline{3-5} 
                                             &                                                                                    & DBL                                                        & \begin{tabular}[c]{@{}l@{}}fuse with core\\ predicate\end{tabular}                                      & the specific action                                                                     \\ \cline{2-5} 
                                             & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}attributes\\ descriptions\end{tabular}} & SBV                                                        & head entity                                                                                             & \begin{tabular}[c]{@{}l@{}}the first entity of\\ the triple\end{tabular}                \\ \cline{3-5} 
                                             &                                                                                    & VOB                                                        & tail entity                                                                                             & \begin{tabular}[c]{@{}l@{}}the second entity of\\ the triple\end{tabular}               \\ \hline
\multirow{8}{*}{SrlT}                        & \multirow{6}{*}{user actions}                                                      & ARG0                                                       & argument1                                                                                               & \begin{tabular}[c]{@{}l@{}}the subject who sends out\\ the specific action\end{tabular} \\ \cline{3-5} 
                                             &                                                                                    & ARG1                                                       & argument2                                                                                               & \begin{tabular}[c]{@{}l@{}}the object undergoing the\\ specific action\end{tabular}     \\ \cline{3-5} 
                                             &                                                                                    & TMP                                                        & time                                                                                                    & \begin{tabular}[c]{@{}l@{}}when does the specific\\ action happen\end{tabular}          \\ \cline{3-5} 
                                             &                                                                                    & LOC                                                        & location                                                                                                & \begin{tabular}[c]{@{}l@{}}where does the specific\\ action happen\end{tabular}         \\ \cline{3-5} 
                                             &                                                                                    & MNR                                                        & manner                                                                                                  & \begin{tabular}[c]{@{}l@{}}how does the specific\\ action happen\end{tabular}           \\ \cline{3-5} 
                                             &                                                                                    & PRP                                                        & reason                                                                                                  & \begin{tabular}[c]{@{}l@{}}why does the specific\\ action happen\end{tabular}           \\ \cline{2-5} 
                                             & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}attributes\\ descriptions\end{tabular}} & ARG0                                                       & head entity                                                                                             & \begin{tabular}[c]{@{}l@{}}the first entity of\\ the triple\end{tabular}                \\ \cline{3-5} 
                                             &                                                                                    & ARG1                                                       & tail entity                                                                                             & \begin{tabular}[c]{@{}l@{}}the second entity of\\ the triple\end{tabular}               \\ \hline
\multicolumn{1}{|l|}{\multirow{9}{*}{SdgpT}} & \multirow{7}{*}{user actions}                                                      & \begin{tabular}[c]{@{}l@{}}AGT\\ EXP\end{tabular}          & argument1                                                                                               & \begin{tabular}[c]{@{}l@{}}the subject who sends out\\ the specific action\end{tabular} \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & \begin{tabular}[c]{@{}l@{}}PAT\\ CONT\end{tabular}         & argument2                                                                                               & \begin{tabular}[c]{@{}l@{}}the object undergoing the\\ specific action\end{tabular}     \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & TIME                                                       & time                                                                                                    & \begin{tabular}[c]{@{}l@{}}when does the specific\\ action happen\end{tabular}          \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & LOC                                                        & location                                                                                                & \begin{tabular}[c]{@{}l@{}}where does the specific\\ action happen\end{tabular}         \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & \begin{tabular}[c]{@{}l@{}}TOOL\\ MATL\\ MANN\end{tabular} & manner                                                                                                  & \begin{tabular}[c]{@{}l@{}}how does the specific\\ action happen\end{tabular}           \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & REAS                                                       & reason                                                                                                  & \begin{tabular}[c]{@{}l@{}}why does the specific\\ action happen\end{tabular}           \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & mNEG                                                       & negation words                                                                                          & words that negate the core predicate                                                    \\ \cline{2-5} 
\multicolumn{1}{|l|}{}                       & \multirow{2}{*}{attributes descriptions}                                           & EXP                                                        & head entity                                                                                             & the first entity of the triple                                                          \\ \cline{3-5} 
\multicolumn{1}{|l|}{}                       &                                                                                    & LINK                                                       & tail entity                                                                                             & the second entity of the triple                                                         \\ \hline
\end{tabular}
}
\end{table*}

==> tables/align.tex <==
\begin{table}[t]
    \centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|c|}{Procedure}             & Semantic Dependency \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{agent}} & EXP                 \\ \cline{2-2} 
% \multicolumn{1}{|c|}{}                         & AGT                 \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{patient}}  & PAT                 \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                         & CONT                \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                         & DATV                \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                         & LINK                \\ \hline
time                                           & TIME                \\ \hline
location                                       & LOC                 \\ \hline
\multirow{3}{*}{manner}                        & MANN                \\ \cline{2-2} 
                                               & MATL                \\ \cline{2-2} 
                                               & TOOL                \\ \hline
\multirow{2}{*}{verb mark}                 & mNEG                \\ \cline{2-2} 
                                               & mDEPD               \\ \hline
\end{tabular}
    \caption{The alignment between the labels of procedure and semantic dependency}
    \label{tab:alig_kh}
\end{table}
\begin{table}[t]
    \centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|c|}{Declaration}              & Semantic Dependency   \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{entity}}   & EXP                   \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                          & AGT                   \\ \hline
sub-entity                                      & \multirow{2}{*}{FEAT} \\ \cline{1-1}
property                                        &                       \\ \hline
property                                        & Belg                  \\ \hline
property value                                 & Clas                  \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{patient}} & PAT                   \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                          & CONT                  \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                          & DATV                  \\ \cline{2-2} 
\multicolumn{1}{|c|}{}                          & LINK                  \\ \hline
time                                            & TIME                  \\ \hline
location                                        & LOC                   \\ \hline
\multirow{3}{*}{manner}                         & MANN                  \\ \cline{2-2} 
                                                & MATL                  \\ \cline{2-2} 
                                                & TOOL                  \\ \hline
cause                                           & REAS                  \\ \hline
\multirow{2}{*}{verb mark}                  & mNEG                  \\ \cline{2-2} 
                                            & mDEPD                 \\ \hline
\end{tabular}
    \caption{The alignment between the labels of declaration and semantic dependency}
    \label{tab:alig_kt}
\end{table}
